Forward-backward envelope for the sum of two nonconvex functions: Further properties and nonmonotone line-search algorithms

We propose ZeroFPR, a nonmonotone linesearch algorithm for minimizing the sum of two nonconvex functions, one of which is smooth and the other possibly nonsmooth. ZeroFPR is the first algorithm that, despite being fit for fully nonconvex problems and requiring only the black-box oracle of forward-backward splitting (FBS) --- namely evaluations of the gradient of the smooth term and of the proximity operator of the nonsmooth one --- achieves superlinear convergence rates under mild assumptions at the limit point when the linesearch directions satisfy a Dennis-Mor\'e condition, and we show that this is the case for quasi-Newton directions. Our approach is based on the forward-backward envelope (FBE), an exact and strictly continuous penalty function for the original cost. Extending previous results we show that, despite being nonsmooth for fully nonconvex problems, the FBE still enjoys favorable first- and second-order properties which are key for the convergence results of ZeroFPR. Our theoretical results are backed up by promising numerical simulations. On large-scale problems, by computing linesearch directions using limited-memory quasi-Newton updates our algorithm greatly outperforms FBS and its accelerated variant (AFBS).

==> TeX/Alg/zerofpr_nonadaptive.tex <==
\begin{algorithmic}[1]
\item[]%
	\renewcommand\arraystretch{1.2}%
	\setlength\tabcolsep{2pt}%
	\renewcommand\myVar\quad%
	\begin{tabularx}{\linewidth}[t]{|>$l<$ @\myVar >$r<$ >$c<$ >$l<$ @\myVar >$r<$ >$c<$ >$l<$ @\myVar >$r<$ >$c<$ >$l<$ X|}
		\hline
		\text{\bf Require} &
			x^0 &\in& \R^n &
			\gamma&\in& (0,\min\set{\nicefrac{1}{L_f},\gamma_g}) &
			\alpha,\beta,p_{\rm min} &\in& (0,1) &
		\\ &
			&&&
			\sigma&\in& (0,\frac{1-\gamma L_f}{2\gamma}) &
			\seq{p_k}&\subset& [p_{\rm min},1] &
		\\[2pt]
		\hline
		\text{\bf Initialize} &
			k &=& 0 &
			\bar\Phi_0 &=& \varphi_\gamma(x^0) &
			&&&
		\\\hline
	\end{tabularx}%
	\vspace{2pt}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\STATE\label{state:zerofpr_nonadaptive:Initial}%
	Select \(\bar x^k\in T_{\gamma}(x^k)\) ~and set~ \(r^k=x^k-\bar x^k\)%
%%%%
\STATE\label{state:zerofpr_nonadaptive:Stop}%
	{\bf if}~ \(\|r^k\|=0\), ~{\bf then}~ stop; ~{\bf end if}%
%%%%
\STATE%
	Select a direction \(d^k\in\R^n\)%
%%%%
\STATE\label{state:zerofpr_nonadaptive:LS}%
	Let \(\tau_k = \beta^{m}\) with \(m\in\N\) being the smallest such that
	\vspace{-0.5\baselineskip}%
	\[
			\varphi_\gamma(\bar x^k + \tau_kd^k)
		{}\leq{}
			\bar\Phi_k
			{}-{}
			\sigma
			\|r^k\|^2
	\]\vspace{-1.25\baselineskip}%
%%%%
	\renewcommand\myVar{\bar\Phi_{k+1}}%
\STATE%
	\(
		\fillwidthof[l]\myVar{x^{k+1}}
	{}={}
		\bar x^k + \tau_kd^k
	\)%
%%%%
\STATE\label{state:zerofpr_nonadaptive:nm}%
	\(
		\fillwidthof[l]\myVar{\bar\Phi_{k+1}}
	{}={}
		(1-p_k)\bar\Phi_k
		{}+{}
		p_k\varphi_\gamma(x^{k+1})
	\)%
%%%%
\item[]%
	\(
		k
	{}\gets{}
		k+1
	\)~
	and go to step \ref{state:zerofpr_nonadaptive:Initial}.%
\end{algorithmic}


















==> TeX/Tables/table_MaxCut.tex <==
\begin{tabular}{|@{\,}lHH@{\,}|l@{\,}|HrHHl@{\,}|HHHHHHrHHl@{\,}|@{\,}}
%\hline
%& & & \multicolumn{2}{c|}{Fast FBS} & \multicolumn{2}{c|}{L-BFGS} & \multicolumn{2}{c|}{Alg.~\ref{alg:GlobalFixed} (L-BFGS)} \\
%ID  & $\lambda/\lambda_\max$ & nnz($x^\star$) & iterations & matvecs & iterations & matvecs & iterations & matvecs \\
%\hline
%\hline
\hline
		&		&		&		&
		\multicolumn{5}{c|}{FBS} 								&
		\multicolumn{5}{H}{L-Broyden}				&
		\multicolumn{5}{c|}{L-BFGS} \\
Graph	& nodes & edges & tol	& it	& $\nabla f$ & $\prox_g$ & obj & avg. cut	& it & $\nabla f$ & $\prox_g$ & obj & avg. cut	& it & $\nabla f$ & $\prox_g$ & obj & avg. cut \\
\hline
%G67 & 10000 & 20000 & $10^{-1}$ &
%	12 &    24 &    12 & 7.47044956$\cdot 10^3$ & 5.7141$\cdot 10^3$ &
%	6 &    17 &    11 & 7.51284136$\cdot 10^3$ & 5.7820$\cdot 10^3$ &
%	6 &    17 &    11 & 7.57200921$\cdot 10^3$ & 5.8796$\cdot 10^3$ \\
%$n=10000$ & 10000 & 20000 & $10^{-2}$ &
%	104 &   208 &   104 & 7.71484731$\cdot 10^3$ & 6.1348$\cdot 10^3$ &
%	24 &    71 &    47 & 7.72155590$\cdot 10^3$ & 6.1507$\cdot 10^3$ &
%	40 &   119 &    79 & 7.73776621$\cdot 10^3$ & 6.1862$\cdot 10^3$ \\
% & 10000 & 20000 & $10^{-3}$ &
%	779 &  1558 &   779 & 7.74058237$\cdot 10^3$ & 6.1923$\cdot 10^3$ &
%	130 &   389 &   259 & 7.74317250$\cdot 10^3$ & 6.2016$\cdot 10^3$ &
%	248 &   744 &   496 & 7.74422154$\cdot 10^3$ & 6.2046$\cdot 10^3$ \\
% & 10000 & 20000 & $10^{-4}$ &
%	8402 & 16804 &  8402 & 7.74408803$\cdot 10^3$ & 6.2026$\cdot 10^3$ &
%	708 &  2123 &  1415 & 7.74438583$\cdot 10^3$ & 6.2051$\cdot 10^3$ &
%	780 &  2340 &  1560 & 7.74443105$\cdot 10^3$ & 6.2036$\cdot 10^3$ \\
%	\hline
%G70 & 10000 & 9999 & $10^{-1}$ &
%	15 &    30 &    15 & 9.63243192$\cdot 10^3$ & 8.9192$\cdot 10^3$ &
%	7 &    20 &    13 & 9.66940799$\cdot 10^3$ & 8.9902$\cdot 10^3$ &
%	7 &    20 &    13 & 9.71342468$\cdot 10^3$ & 9.0694$\cdot 10^3$ \\
%$n=10000$ & 10000 & 9999 & $10^{-2}$ &
%	108 &   216 &   108 & 9.82664257$\cdot 10^3$ & 9.3288$\cdot 10^3$ &
%	30 &    89 &    59 & 9.83946898$\cdot 10^3$ & 9.3612$\cdot 10^3$ &
%	68 &   204 &   136 & 9.86027967$\cdot 10^3$ & 9.4271$\cdot 10^3$ \\
% & 10000 & 9999 & $10^{-3}$ &
%	977 &  1954 &   977 & 9.86072737$\cdot 10^3$ & 9.4309$\cdot 10^3$ &
%	117 &   350 &   233 & 9.86129707$\cdot 10^3$ & 9.4340$\cdot 10^3$ &
%	126 &   378 &   252 & 9.86150243$\cdot 10^3$ & 9.4353$\cdot 10^3$ \\
% & 10000 & 9999 & $10^{-4}$ &
%	3059 &  6118 &  3059 & 9.86149280$\cdot 10^3$ & 9.4352$\cdot 10^3$ &
%	244 &   731 &   487 & 9.86151961$\cdot 10^3$ & 9.4352$\cdot 10^3$ &
%	225 &   675 &   450 & 9.86152361$\cdot 10^3$ & 9.4348$\cdot 10^3$ \\
%% & 10000 & 9999 & 1.0e-05 &
%%	12693 & 25386 & 12693 & 9.86152331$\cdot 10^3$ & 9.4365$\cdot 10^3$ &
%%	449 &  1346 &   897 & 9.86152381$\cdot 10^3$ & 9.4352$\cdot 10^3$ &
%%	290 &   870 &   580 & 9.86152386$\cdot 10^3$ & 9.4367$\cdot 10^3$ \\
%\hline
G72 & 10000 & 20000 & $10^{-1}$ &
	11 &    22 &    11 & 7.51199253$\cdot 10^3$ & 5.7436$\cdot 10^3$ &
	6 &    17 &    11 & 7.57964723$\cdot 10^3$ & 5.8499$\cdot 10^3$ &
	6 &    17 &    11 & 7.63835469$\cdot 10^3$ & 5.9479$\cdot 10^3$ \\
$n=10000$ & 10000 & 20000 & $10^{-2}$ &
	104 &   208 &   104 & 7.77880446$\cdot 10^3$ & 6.1914$\cdot 10^3$ &
	23 &    68 &    45 & 7.78360233$\cdot 10^3$ & 6.2019$\cdot 10^3$ &
	34 &   101 &    67 & 7.79955282$\cdot 10^3$ & 6.2381$\cdot 10^3$ \\
 & 10000 & 20000 & $10^{-3}$ &
	837 &  1674 &   837 & 7.80487444$\cdot 10^3$ & 6.2514$\cdot 10^3$ &
	126 &   377 &   251 & 7.80714572$\cdot 10^3$ & 6.2552$\cdot 10^3$ &
	207 &   620 &   413 & 7.80827806$\cdot 10^3$ & 6.2625$\cdot 10^3$ \\
 & 10000 & 20000 & $10^{-4}$ &
	7825 & 15650 &  7825 & 7.80816781$\cdot 10^3$ & 6.2578$\cdot 10^3$ &
	613 &  1838 &  1225 & 7.80846818$\cdot 10^3$ & 6.2641$\cdot 10^3$ &
	901 &  2702 &  1801 & 7.80853745$\cdot 10^3$ & 6.2616$\cdot 10^3$ \\
% & 10000 & 20000 & 1.0e-05 &
%	20000 & 40000 & 20000 & 7.80841445$\cdot 10^3$ & 6.2621$\cdot 10^3$ &
%	2269 &  6806 &  4537 & 7.80853709$\cdot 10^3$ & 6.2588$\cdot 10^3$ &
%	1303 &  3909 &  2606 & 7.80853910$\cdot 10^3$ & 6.2613$\cdot 10^3$ \\
\hline
G77 & 14000 & 28000 & $10^{-1}$ &
	11 &    22 &    11 & 1.06229511$\cdot 10^4$ & 8.1506$\cdot 10^3$ &
	6 &    17 &    11 & 1.07182828$\cdot 10^4$ & 8.3004$\cdot 10^3$ &
	6 &    17 &    11 & 1.08022701$\cdot 10^4$ & 8.4333$\cdot 10^3$ \\
$n=14000$ & 14000 & 28000 & $10^{-2}$ &
	106 &   212 &   106 & 1.10041849$\cdot 10^4$ & 8.7927$\cdot 10^3$ &
	24 &    71 &    47 & 1.10127115$\cdot 10^4$ & 8.8082$\cdot 10^3$ &
	42 &   125 &    83 & 1.10365171$\cdot 10^4$ & 8.8632$\cdot 10^3$ \\
 & 14000 & 28000 & $10^{-3}$ &
	892 &  1784 &   892 & 1.10405809$\cdot 10^4$ & 8.8700$\cdot 10^3$ &
	128 &   383 &   255 & 1.10435753$\cdot 10^4$ & 8.8808$\cdot 10^3$ &
	282 &   846 &   564 & 1.10453838$\cdot 10^4$ & 8.8909$\cdot 10^3$ \\
 & 14000 & 28000 & $10^{-4}$ &
	8571 & 17142 &  8571 & 1.10451052$\cdot 10^4$ & 8.8857$\cdot 10^3$ &
	692 &  2075 &  1383 & 1.10455884$\cdot 10^4$ & 8.8888$\cdot 10^3$ &
	956 &  2868 &  1912 & 1.10456717$\cdot 10^4$ & 8.8861$\cdot 10^3$ \\
% & 14000 & 28000 & 1.0e-05 &
%	20000 & 40000 & 20000 & 1.10454564$\cdot 10^4$ & 8.8872$\cdot 10^3$ &
%	2586 &  7757 &  5171 & 1.10456747$\cdot 10^4$ & 8.8847$\cdot 10^3$ &
%	1611 &  4833 &  3222 & 1.10456773$\cdot 10^4$ & 8.8875$\cdot 10^3$ \\
\hline
G81 & 20000 & 40000 & $10^{-1}$ &
	11 &    22 &    11 & 1.50520470$\cdot 10^4$ & 1.1511$\cdot 10^4$ &
	6 &    17 &    11 & 1.51888877$\cdot 10^4$ & 1.1723$\cdot 10^4$ &
	6 &    17 &    11 & 1.53078128$\cdot 10^4$ & 1.1918$\cdot 10^4$ \\
$n=20000$ & 20000 & 40000 & $10^{-2}$ &
	93 &   186 &    93 & 1.55886305$\cdot 10^4$ & 1.2410$\cdot 10^4$ &
	24 &    71 &    47 & 1.56090268$\cdot 10^4$ & 1.2453$\cdot 10^4$ &
	38 &   113 &    75 & 1.56407133$\cdot 10^4$ & 1.2522$\cdot 10^4$ \\
 & 20000 & 40000 & $10^{-3}$ &
	1142 &  2284 &  1142 & 1.56504523$\cdot 10^4$ & 1.2548$\cdot 10^4$ &
	144 &   431 &   287 & 1.56537865$\cdot 10^4$ & 1.2558$\cdot 10^4$ &
	326 &   978 &   652 & 1.56558923$\cdot 10^4$ & 1.2562$\cdot 10^4$ \\
 & 20000 & 40000 & $10^{-4}$ &
	8884 & 17768 &  8884 & 1.56554466$\cdot 10^4$ & 1.2562$\cdot 10^4$ &
	769 &  2306 &  1537 & 1.56560722$\cdot 10^4$ & 1.2564$\cdot 10^4$ &
	1012 &  3036 &  2024 & 1.56561816$\cdot 10^4$ & 1.2570$\cdot 10^4$ \\
% & 20000 & 40000 & 1.0e-05 &
%	20000 & 40000 & 20000 & 1.56558694$\cdot 10^4$ & 1.2565$\cdot 10^4$ &
%	3004 &  9011 &  6007 & 1.56561899$\cdot 10^4$ & 1.2562$\cdot 10^4$ &
%	2223 &  6669 &  4446 & 1.56561945$\cdot 10^4$ & 1.2566$\cdot 10^4$ \\
\hline
\end{tabular}



==> TeX/Tables/table_lasso.tex <==
\setlength\tabcolsep{5.5pt}
\begin{tabular}{|@{}|l|r|r||rr|HHrr|@{}}
\hline
& & & \multicolumn{2}{c|}{Fast FBS} & \multicolumn{2}{H}{L-Broyden} & \multicolumn{2}{c|}{L-BFGS} \\
ID  & $\lambda/\lambda_{\max}$ & nnz($x^\star$) & iterations & matvecs & iterations & matvecs & iterations & matvecs \\
\hline
\hline
\textbf{191} & $1\cdot 10^{-1}$		& 3  & 2260 &   4520 & 334 &   1334 & 125 &    498  \\
$m=8192$ & $5\cdot 10^{-2}$			& 4  & 7529  & 15058 & 828 &   3310 &    276 &   1102 \\
$n=32768$ & $1\cdot 10^{-2}$		& 7  & 11222 & 22444 & 1768 &   7070 &   592 &   2366 \\
\hline
\textbf{192} & $9\cdot 10^{-1}$		& 2  & 234   & 468   & 3 & 10 & 3   & 10    \\
$m=8192$ & $7\cdot 10^{-1}$			& 9  & 649   & 1298  & 48 &    190 &  28 &    110  \\
$n=32768$ & $5\cdot 10^{-1}$		& 21 & 2051  & 4102  & 813 &   3250 &    120 &    478  \\
\hline
\textbf{193} & $5\cdot 10^{-1}$		& 3  & 2142  & 4284  & 417 &   1666 & 182 &    726  \\
$m=8192$ & $1\cdot 10^{-1}$			& 4  & 2413  & 4826  & 839 &   3354 &    479 &   1914 \\
$n=32768$ & $5\cdot 10^{-2}$		& 5  & 4761  & 9522  & 1308 &   5230 &    642 &   2566 \\
\hline
\textbf{194} & $9\cdot 10^{-1}$		& 6  & 338   & 676   & 32 &    126 &     16 &     62   \\
$m=8192$ & $7\cdot 10^{-1}$			& 29 & 1532  & 3064  & 204 &    814 &    223 &    890  \\
$n=32768$ & $5\cdot 10^{-1}$		& 51 & 2482  & 4964  & 538 &   2150 &    385 &   1538 \\
\hline
\textbf{195} & $5\cdot 10^{-2}$		& 2  & 3215  & 6430  & 605 &   2418 &    164 &    654  \\
$m=8192$ & $1\cdot 10^{-2}$			& 3  & 3833  & 7666  & 2225 &   8898 &    458 &   1830 \\
$n=32768$ & $5\cdot 10^{-3}$		& 4  & 10525 & 21050 & 3549 &  14194 & 688 &   2750 \\
\hline
\textbf{196} & $7\cdot 10^{-1}$		& 2  & 651   & 1302  & 21 &     82 &    12 &     46   \\
$m=8192$ & $5\cdot 10^{-1}$			& 4  & 1656  & 3312  & 82 &    326 &     28 &    110  \\
$n=32768$ & $1\cdot 10^{-1}$		& 11 & 3075  & 6150  & 766 &   3062 &     395 &   1578 \\
\hline
\textbf{197} & $1\cdot 10^{-1}$		& 3  & 3863  & 7726  & 491 &   1962 &    349 &   1394 \\
$m=8192$ & $5\cdot 10^{-2}$			& 4  & 4343  & 8686  & 807 &   3226 &    483 &   1930 \\
$n=32768$ & $1\cdot 10^{-2}$		& 6  & 10894 & 21788 & 2728 &  10910 &   1397 &   5586 \\
\hline
\textbf{198} & $9\cdot 10^{-1}$		& 4  & 628   & 1256  & 45 &    178 &     49 &    194   \\
$m=8192$ & $7\cdot 10^{-1}$			& 17 & 2351  & 4702  & 109 &    434 &    219 &    874  \\
$n=32768$ & $5\cdot 10^{-1}$		& 25 & 3236  & 6472  & 262 &   1046 &    252 &   1006  \\
\hline
\textbf{199} & $1\cdot 10^{-1}$		& 2  & 7163  & 14326 & 705 &   2818 &    338 &   1350 \\
$m=8192$ & $5\cdot 10^{-2}$			& 3  & 2537  & 5074  & 1301 &   5202 &    554 &   2214 \\
$n=49152$ & $1\cdot 10^{-2}$		& 5  & 10460 & 20920 & 3174 &  12694 &   1271 &   5082 \\
\hline
\textbf{200} & $9\cdot 10^{-1}$		& 6  & 622   & 1244  & 73 &    290 &     71 &    282  \\
$m=8192$ & $7\cdot 10^{-1}$			& 10 & 2144  & 4288  & 200 &    798 &    166 &    662  \\
$n=49152$ & $5\cdot 10^{-1}$		& 19 & 2313  & 4626  & 324 &   1294 &    298 &   1190 \\
\hline
\end{tabular}



==> TeX/Tables/table_lasso_err.tex <==
\setlength\tabcolsep{5.5pt}
\begin{tabular}{|@{}|l|r|r||rr|rr|@{}}
\hline
& & & \multicolumn{2}{c|}{Fast FBS} & \multicolumn{2}{c|}{L-BFGS} \\
ID  & $\lambda/\lambda_{\max}$ & nnz($x^\star$) & iterations & matvecs & iterations & matvecs \\
\hline
\hline
\textbf{191} & $1\cdot 10^{-1}$		& 3  & 5275  & 10550 & 126  & 502  \\
$m=8192$ & $5\cdot 10^{-2}$			& 4  & 10232 & 20464 & 273  & 1090 \\
$n=32768$ & $1\cdot 10^{-2}$		& 7  & 12211 & 24422 & 546  & 2182 \\
\hline
\textbf{192} & $9\cdot 10^{-1}$		& 2  & 651   & 1302  & 3    & 10   \\
$m=8192$ & $7\cdot 10^{-1}$			& 9  & 6293  & 12586 & 51   & 202  \\
$n=32768$ & $5\cdot 10^{-1}$		& 21 & 10514 & 21028 & 131  & 522  \\
\hline
\textbf{193} & $5\cdot 10^{-1}$		& 3  & 7532  & 15064 & 209  & 834  \\
$m=8192$ & $1\cdot 10^{-1}$			& 4  & 5748  & 11496 & 491  & 1962 \\
$n=32768$ & $5\cdot 10^{-2}$		& 5  & 8076  & 16152 & 606  & 2422 \\
\hline
\textbf{194} & $9\cdot 10^{-1}$		& 6  & 7332  & 14664 & 28   & 110  \\
$m=8192$ & $7\cdot 10^{-1}$			& 29 & 9657  & 19314 & 257  & 1026 \\
$n=32768$ & $5\cdot 10^{-1}$		& 51 & 9503  & 19006 & 452  & 1806 \\
\hline
\textbf{195} & $5\cdot 10^{-2}$		& 2  & 5636  & 11272 & 172  & 686  \\
$m=8192$ & $1\cdot 10^{-2}$			& 3  & 3857  & 7714  & 438  & 1750 \\
$n=32768$ & $5\cdot 10^{-3}$		& 4  & 8026  & 16052 & 708  & 2830 \\
\hline
\textbf{196} & $7\cdot 10^{-1}$		& 2  & 5283  & 10566 & 16   & 62   \\
$m=8192$ & $5\cdot 10^{-1}$			& 4  & 7092  & 14184 & 30   & 118  \\
$n=32768$ & $1\cdot 10^{-1}$		& 11 & 7313  & 14626 & 415  & 1658 \\
\hline
\textbf{197} & $1\cdot 10^{-1}$		& 3  & 7686  & 15372 & 330  & 1318 \\
$m=8192$ & $5\cdot 10^{-2}$			& 4  & 6851  & 13702 & 571  & 2282 \\
$n=32768$ & $1\cdot 10^{-2}$		& 6  & 9946  & 19892 & 1328 & 5310 \\
\hline
\textbf{198} & $9\cdot 10^{-1}$		& 4  & 10301 & 20602 & 78   & 310  \\
$m=8192$ & $7\cdot 10^{-1}$			& 17 & 14034 & 28068 & 217  & 866  \\
$n=32768$ & $5\cdot 10^{-1}$		& 25 & 13626 & 27252 & 272  & 1086 \\
\hline
\textbf{199} & $1\cdot 10^{-1}$		& 2  & 12641 & 25282 & 328  & 1310 \\
$m=8192$ & $5\cdot 10^{-2}$			& 3  & 4953  & 9906  & 620  & 2478 \\
$n=49152$ & $1\cdot 10^{-2}$		& 5  & 12949 & 25898 & 1356 & 5422 \\
\hline
\textbf{200} & $9\cdot 10^{-1}$		& 6  & 10281 & 20562 & 87   & 346  \\
$m=8192$ & $7\cdot 10^{-1}$			& 10 & 13619 & 27238 & 211  & 842  \\
$n=49152$ & $5\cdot 10^{-1}$		& 19 & 10763 & 21526 & 327  & 1306 \\
\hline
\end{tabular}



==> TeX/Text/Simulations/Lasso.tex <==
The problem is to find a sparse least square solution to a system which is usually
underdetermined. This is done by minimizing $\varphi = f+g$ where
$$ f(x) = \tfrac{1}{2}\|Ax-b\|_2^2,\quad g(x) = \lambda\|x\|_1, $$
and $A\in\R^{m\times n}$ and $b\in\R^m$.
In this case $g$ is convex, and its (single-valued) proximal mapping is the soft-thresholding operation.
%$$ \prox_{\gamma g}(x) = \sign(x)\max\{0,|x|-\lambda\gamma\}, $$
The computationally relevant operation here is the computation of $f$ and $\nabla f$, which
involves matrix-vector products with $A$ and $\trans A$.
Parameter $\lambda$ modulates between a small residual
$Ax^\star-b$ and a sparse solution vector $x^\star$, \ie, the larger $\lambda$ the
more zero coefficients $x^\star$ has. In particular, $\lambda_{\max} = \|\trans A b\|_\infty$
is the minimum value such that for $\lambda \geq \lambda_{\max}$ the solution is $x^\star = 0$.
We have $L_f = \|\trans A A\|$, which can be quickly approximated using power iterations.

We ran the algorithms on the SPEAR datasets.\footnote{\url{http://wwwopt.mathematik.tu-darmstadt.de/spear/}}
First we considered Broyden and BFGS directions in \Cref{alg:zerofpr} on small dimensional instances, and the results are
illustrated in \Cref{fig:LassoSmall}.
We computed $x^\star$ (approximately) by running
one of the methods with very restrictive termination criteria.
Then we considered the largest instances implementing L-BFGS directions in \Cref{alg:zerofpr}.
Performance of the algorithms is detailed in \Cref{tbl:Lasso}.
It is apparent that \Cref{alg:zerofpr} requires much less iterations and operations than fast FBS.

%\begin{figure}
%\centering
%	\input{TeX/Tikz/spear_1_matvecs_vs_distance.tex}%
%	\input{TeX/Tikz/spear_1_matvecs_vs_FPR.tex}		
%\caption{Lasso: performance of the methods on the
%	\texttt{spear\_inst\_1} dataset, with $n=1024$ and $m=512$, for
%	$\lambda = 0.2\lambda_{\max}$.}
%\end{figure}

\begin{figure}
\centering
%	\begin{subfigure}{0.49\textwidth}
%		\includetikz[width=\linewidth]{spear_inst_1_lam_0_1_matvecs_vs_distance}
%		\caption{\texttt{spear\_inst\_1}}
%	\end{subfigure}\hfill
%	\begin{subfigure}{0.49\textwidth}
%		\includetikz[width=\linewidth]{spear_inst_2_lam_0_1_matvecs_vs_distance}
%		\caption{\texttt{spear\_inst\_2}}
%	\end{subfigure}
%	
%	\vspace{1cm}
%	\begin{subfigure}{0.49\textwidth}
%		\includetikz[width=\linewidth]{spear_inst_3_lam_0_1_matvecs_vs_distance}
%		\caption{\texttt{spear\_inst\_3}}
%	\end{subfigure}\hfill
%	\begin{subfigure}{0.49\textwidth}
%		\includetikz[width=\linewidth]{spear_inst_4_lam_0_1_matvecs_vs_distance}
%		\caption{\texttt{spear\_inst\_4}}
%	\end{subfigure}
%	
%	\vspace{1cm}
%	\begin{subfigure}{0.49\textwidth}
%		\includetikz[width=\linewidth]{spear_inst_5_lam_0_1_matvecs_vs_distance}
%		\caption{\texttt{spear\_inst\_5}}
%	\end{subfigure}\hfill
%	\begin{subfigure}{0.49\textwidth}
		\includetikz[width=0.7\linewidth]{spear_inst_6_lam_0_1_matvecs_vs_distance}
%		\caption{\texttt{spear\_inst\_6}}
%	\end{subfigure}
\caption{Lasso: performance
	\siam{%
		of the methods
	}%
	on the
	\texttt{spear\_inst\_6} dataset, with $n=1024$ and $m=512$, for
	$\lambda = 0.1\lambda_{\max}$. On the $x$-axis is the number of matrix-vector products computed,
	on the $y$-axis is the relative error $\|x^k-x^\star\|_{\infty}/\|x^\star\|_{\infty}$.
%	In \Cref{alg:zerofpr} we used BFGS and modified Broyden with nonmonotone linesearch.
}\label{fig:LassoSmall}
\end{figure}

\begin{table}[tb]
\tiny
\centering
\input{TeX/Tables/table_lasso.tex}
\caption{Lasso: performance of the algorithms
on the largest of the considered datasets. Column ID indicates the identification number of
the dataset among the SPEAR instances.
Results refer to iterations and matrix vector
products needed to obtain $(\varphi(x^k)-\varphi_\star)/|\varphi_\star| \leq 10^{-6}$.
%In \Cref{alg:zerofpr} we used L-BFGS directions with nonmonotone linesearch.
}\label{tbl:Lasso}
\end{table}


==> TeX/Text/Simulations/MatrixCompletion.tex <==
%We consider the problem of recovering the entries of an $m$-by-$n$ matrix, which is known to have small rank, from a sample of them.
%One may refer to~\cite{candes2009exact} for a detailed theoretical analysis of the problem.
%The decision variable is now a matrix $X = (x_{ij})\in\R^{m\times n}$, and
The problem has the form
\begin{align*}
\minimize_{X\in\R^{m\times n}}\ & \tfrac{1}{2}\|\mathcal{A}(X)-b\|^2 \\
\stt\ & \rank(X) \leq r
\end{align*}
%$$f(x) = \tfrac{1}{2}\|\mathcal{A}(x)-b\|^2,\qquad g(x) = \lambda\|x\|_*,$$
where $\mathcal{A}:\R^{m\times n}\to\R^k$ is a linear mapping.
Specifically, $\mathcal{A}$ selects $k$ entries from its matrix arguments and the goal is to find a low-rank matrix given an incomplete measurement of its coefficients.
This problem has application, for example, in recommendation system.
The set of matrices of rank at most $r$ is nonconvex and closed, and the projection onto it is given by %the following operation:
%\begin{equation}\label{eq:ProjRankBall}
	\[\proj_{\rank \leq r}(X) {}={} U_r \diag(\sigma_1, \ldots, \sigma_r) V_r^T.\]
%\end{equation}
Here, $\sigma_1\ldots \sigma_r$ are $r$ largest singular values of $X$, and $U_r, V_r$ are the matrices
%having as columns the correspondent
of left and right singular vectors, respectively: each computation of $\Pi_{\rank \leq r}$ entails
the computation of a partial SVD which is, from the most computational perspective, the significantly expensive operation in this case. In our implementations we have used MATLAB's \texttt{svds} to perform the projection.
We ran the methods
%compared FBS with \Cref{alg:zerofpr} using L-BFGS directions,
on the MovieLens100k dataset.\footnote{\url{http://grouplens.org/datasets/movielens/}}
This consists of $10^5$ ratings of $1682$ movies
from $943$ users, so the problem has $\approx 1.6$ millions variables.
The results are in \Cref{fig:matcomp1}.

\begin{figure}[tbp]
\centering
\begin{subfigure}{0.43\textwidth}
	\includetikz[width=\linewidth]{MatComp/MatComp_5}\hfill
	\caption{$r = 5$}
\end{subfigure}
\begin{subfigure}{0.43\textwidth}
	\includetikz[width=\linewidth]{MatComp/MatComp_15}
	\caption{$r = 15$}
\end{subfigure}
\caption{Matrix completion: convergence of the cost in FBS and \Cref{alg:zerofpr} with L-BFGS directions, for $r = 5, 15$.
%The methods are compared in terms of number of (partial) SVDs vs. decrease in the objective value.
}\label{fig:matcomp1}
\end{figure}

%vector $b\in\Re^k$ contains the known entries, and $\|x\|_*$ indicates the nuclear norm of $x$, which is the sum of its singular values.
%%Indicating with $r$ the rank of $x$, the proximal mapping associated with $g$ is the following
%%singular value thresholding operation:
%%$$ \prox_{\gamma g}(x) = U \Sigma_+ V^T, \quad \Sigma_+ = \diag(\max\{0, \sigma_i-\gamma\lambda\}, i=1\ldots r), $$
%In this case $L_f=1$, therefore we can apply \Cref{alg:GlobalFixed}.
%
%The most computational expensive operation here is the proximal step,
%requiring the computation of a SVD.
%Computing the full SVD becomes computationally infeasible as $m$ and $n$ grow, therefore we use
%the following partial decomposition strategy in computing the proximal mapping: start with $\nu_0 = 10$, and
%the $i$-th time $\prox_{\gamma g}$ is evaluated compute only the largest $\nu_i$ singular values $\sigma_1\geq\ldots\geq\sigma_{\nu_i}$, and
%$$ \prox_{\gamma g}(x) \approx U \tilde{\Sigma}_+ V^T, \quad \tilde{\Sigma}_+ = \diag(\max\set{0, \sigma_i-\gamma\lambda}, i=1\ldots \nu_i), $$
%Then set $\nu_{i+1}$ according to the following rule
%$$ \nu_{i+1} = \begin{cases}
%  \min\set{j}{\sigma_j \leq \gamma} & \mbox{if } \sigma_{\nu_i} \leq \gamma\lambda \\
%  \nu_i + 5 & \mbox{otherwise.}
%\end{cases}$$
%The same technique for approximately evaluating the singular value thresholing is used in other algorithms
%for nuclear norm regularization problems \cite{toh2010accelerated}.
%The partial singular value decompositions were performed using PROPACK software package.\footnote{\url{http://sun.stanford.edu/~rmunk/PROPACK/}}
%
%We compared \Cref{alg:GlobalFixed} with L-BFGS directions, classical L-BFGS and FBS
%on the MovieLens100k dataset.\footnote{\url{http://grouplens.org/datasets/movielens/}} This consists of $10^5$ ratings of $1682$ movies
%from $943$ users, so that the problem has $\approx 1.6$ millions variables. The results of the simulations, for decreasing values of $\lambda$, are in \Cref{fig:MatComp1}.


==> TeX/Text/Simulations/MaxCut.tex <==
Let \(G = (V, E)\) be an undirected weighted graph, with \(n=|V|\) nodes. The weights of the edges \(E\) are collected in a (symmetric) matrix
$W = (w_{ij})\in\R^{n\times n}$, so that \(w_{ij} = 0\) whenever \((i,j)\notin E\).
We want to partition (\emph{cut}) the nodes
into two subsets so that the sum of the weights of the edges connecting the two subsets is maximized.
A cut can be represented as a combination of \(x_1,\ldots,x_n\in\{0,1\}\), and the total weight of the edges connecting the two subsets (the \emph{cut value}) can be computed as \(\sum_{i<j}w_{ij}(1-x_ix_j)\). Therefore, we want to solve

\begin{equation}\label{eq:MaxCut}
	\maximize_{x_1,\ldots,x_n\in\{0,1\}}\ \sum_{i<j}w_{ij}(1-x_ix_j).
\end{equation}

This is a hard combinatorial problem.
In \cite{goemans1995improved} they propose an approximation algorithm, which consists of solving an SDP relaxation to \eqref{eq:MaxCut}:
from the solution to such SDP, random cuts (\ie, random assignements of the nodes to the two subsets) can be generated such that their average value is at least \(0.87856\) times the optimal cut value, see \cite[Lem. 3.5]{goemans1995improved}.

The authors of \cite{burer2003nonlinear} propose instead to solve the following nonconvex but considerably smaller problem:
\begin{equation}
\begin{aligned}\label{eq:BurerMonteiroZhangRelaxation}
	\minimize_{x_1\ldots x_n\in\mathcal{S}^r}\ & \sum_{i<j} w_{ij}\innprod{x_i}{x_j}, % \\
%	\stt\ 							& \|x_i\| = 1,\ i=1\ldots n
\end{aligned}
\end{equation}
where $\mathcal{S}^r$ denotes the unit sphere in $\R^r$.
%Provided that $r$ is large enough, problem \eqref{eq:BurerMonteiroZhangRelaxation} is equivalent to the
%SDP relaxation by Goemans and Williamson \cite{goemans1995improved}.
Provided that $r$ is sufficiently large, \eqref{eq:BurerMonteiroZhangRelaxation} is equivalent to the SDP relaxation of \cite{goemans1995improved}.
From a solution to \eqref{eq:BurerMonteiroZhangRelaxation}, a random cut is computed as follows: select a vector $v$ uniformly at random on the unit sphere, then assign each node $i$ to either of the two subsets according to the $\sgn{\innprod{x_i}{v}}$.

%This strategy produces a cut whose average weight is larger than $0.878$ times the optimal.
%Denoting with $\mathcal{S}^n$ the unit sphere in $\R^n$, Goemans and Williamson \cite{goemans1995improved} proposed the following
%relaxation of the above problem:
%\begin{align*}
%	\minimize_{X\in\R^{n\times n}}\ 	&\trace(WX) \\
%	\stt\ 							& X\succeq 0 \\
%									& \diag(X) = 1.
%\end{align*}
%\begin{equation}\label{eq:GoemanWilliamsonRelaxation}
%\begin{aligned}
%	\minimize_{x_1\ldots x_n\in\mathcal{S}^n}\ & \sum_{i<j} w_{ij}\innprod{x_i}{x_j}. %\\
%%	\stt\ 							& \|x_i\| = 1,\ i=1\ldots n
%\end{aligned}
%\end{equation}
%From a solution to \eqref{eq:GoemanWilliamsonRelaxation}, a random cut can be computed selecting a vector $v$ uniformly at random on the unit sphere, and assigning each node $i$
%to either of the two subsets according to the $\sgn{\innprod{x_i}{v}}$. This strategy produces
%a cut whose average weight is larger than $0.878$ times the optimal, and in
%\cite{goemans1995improved} they propose an SDP formulation to solve \eqref{eq:GoemanWilliamsonRelaxation}.
%Burer and Monteiro \cite{burer2003nonlinear} showed that solving the same problem with $x_1\ldots x_n\in\mathcal{S}^r$ and $r\leq n$ is equivalent to the SDP relaxation of Goemans and Williamson, provided that $r$ is large enough:
%%\begin{align*}
%%	\minimize_{X\in\R^{r\times n}}\ 	&\trace(WX^\top X) \\
%%	\stt\ 							& \|x_i\| = 1, i=1\ldots n.
%%\end{align*}
%\begin{equation}
%\begin{aligned}\label{eq:BurerMonteiroZhangRelaxation}
%	\minimize_{x_1\ldots x_n\in\mathcal{S}^r}\ & \sum_{i<j} w_{ij}\innprod{x_i}{x_j}. % \\
%%	\stt\ 							& \|x_i\| = 1,\ i=1\ldots n
%\end{aligned}
%\end{equation}
%Therefore the problem consists of the minimization of a nonconvex smooth objective
%over the direct sum of $n$ unit spheres in $\R^r$.
%We applied our \Cref{alg:zerofpr} with Broyden and BFGS directions to problem \eqref{eq:BurerMonteiroZhangRelaxation}, using $r=5$ and the small \emph{torusg3-8}\footnote{\url{http://dimacs.rutgers.edu/Challenges/Seventh/Instances/}} with $512$ nodes and $1536$ edges.
%The results are depicted in \Cref{fig:maxcut}.
%Then w
We applied \Cref{alg:zerofpr} with L-BFGS to the graphs of the \emph{Gset} dataset\footnote{\url{http://web.stanford.edu/~yyye/yyye/Gset/}} and $r=20$. We considered more and more restrictive termination criteria based on $\|\Res(x^k)\|$, and for each solution obtained we computed the average of $500$ random cuts. The results are shown in \Cref{tbl:maxcut}.

%\begin{figure}
%	\centering
%	\includetikz[width=0.45\linewidth]{toursg3-8_FPR}\hfill
%	\includetikz[width=0.45\linewidth]{toursg3-8_Subopt}
%	\caption{Max-cut: convergence of the methods for the graph \texttt{toursg3-8}, with $n = 512$ and using $r=5$. On the left, convergence of the fixed-point residual.
%		On the right, convergence of the objective value to the optimum (all methods converged to the same objective value).}%
%	\label{fig:maxcut}
%\end{figure}

\begin{table}[tb]
	\switch{%SIAM
		\begin{minipage}[t]{0.56\linewidth}
		\vspace*{0pt}%
		\centering%
		{\tiny\input{TeX/Tables/table_MaxCut.tex}}%
		\end{minipage}
		\hfill
		\begin{minipage}[t]{0.435\linewidth}
%			\vspace*{-0.5\baselineskip}
			\vspace*{-\abovecaptionskip}%
			\caption{Max-cut: comparison between FBS and \Cref{alg:zerofpr} with L-BFGS directions.
				The ``avg. cut'' column shows the average value of $500$ random cuts obtained from the computed solution. We used $r = 20$, and stopped the algorithms when $\|\Res(x^k)\|\leq \text{tol}$.}%
			\label{tbl:maxcut}
		\end{minipage}
	}{%ARXIV
		\centering
		{\tiny\input{TeX/Tables/table_MaxCut.tex}}
		\caption{Max-cut: comparison between FBS and \Cref{alg:zerofpr} with L-BFGS directions.
			The ``avg. cut'' column shows the average value of $500$ random cuts obtained from the computed solution. We used $r = 20$, and stopped the algorithms when $\|\Res(x^k)\|\leq \text{tol}$.}%
		\label{tbl:maxcut}
	}%
\end{table}


==> TeX/Text/Simulations/SparseLogReg.tex <==
This is a convex problem, and the composite objective function consists of
$f(x) = \sum_{i=1}^m\log(1+e^{-b_i\innprod{a_{i}}{x}})$ and $g(x) = \lambda\|x\|_1$.
Here vector $a_i\in\R^n$ contains the features of the $i$-th instance, and $b_i\in\set{-1,1}$ indicates the correspondent class.
The $\ell_1$-regularization enforces sparsity in the solution.
Indicating with $A\in\R^{m\times n}$ the matrix having rows $a_1, a_2, \ldots, a_m$, the optimal solution is $x^\star = 0$ if $\lambda \geq \lambda_{\max}\coloneqq \tfrac{1}{2}\|\trans Ab\|_\infty$.
We ran the algorithms on a series of datasets,\footnote{\url{http://www.csie.ntu.edu.tw/~cjlin/libsvmtools/datasets/}} using full and limited-memory quasi-Newton directions.
The results are displayed in \Cref{fig:SparseLogReg} and \Cref{fig:SparseLogReg2}.

\begin{figure}[tbp]
	\switch{%SIAM
		\begin{minipage}[t]{0.52\linewidth}%
		\vspace*{0pt}%
		\centering%
			\includetikz[width=\linewidth]{w4a_lam_5e-2_matvecs_vs_distance}%
		\end{minipage}\hfill
		\begin{minipage}[t]{0.45\linewidth}%
			\vspace*{-\abovecaptionskip}%
			\caption{%
				Sparse logistic regression: performance of the \texttt{w4a} dataset, with $n = 299$, $m = 6760$, using $\lambda = 0.05\lambda_{\max}$.
				On the $x$-axis is the number of matrix-vector products computed,
				on the $y$-axis is the relative error $\|x^k-x^\star\|_{\infty}/\|x^\star\|_{\infty}$.
			}%
			\label{fig:SparseLogReg}%
		\end{minipage}%
	}{%ARXIV
		\includetikz[width=0.6\linewidth]{w4a_lam_5e-2_matvecs_vs_distance}
		\caption{%
			Sparse logistic regression: performance of the \texttt{w4a} dataset, with $n = 299$, $m = 6760$, using $\lambda = 0.05\lambda_{\max}$.
			On the $x$-axis is the number of matrix-vector products computed,
			on the $y$-axis is the relative error $\|x^k-x^\star\|_{\infty}/\|x^\star\|_{\infty}$.
		}%
		\label{fig:SparseLogReg}
	}%
\end{figure}

\begin{figure}[tbp]
\centering
	\begin{subfigure}{0.33\linewidth}
		\centering
		\includetikz[width=\linewidth]{real-sim_err_1e-2}
		\caption{\texttt{real-sim}}
	\end{subfigure}\hfill
	\begin{subfigure}{0.33\linewidth}
		\centering
		\includetikz[width=\linewidth]{rcv1_err_1e-2}
		\caption{\texttt{rcv1}}
	\end{subfigure}\hfill
	\begin{subfigure}{0.33\linewidth}
		\centering
		\includetikz[width=\linewidth]{news20_err_1e-2}
		\caption{\texttt{news20}}
	\end{subfigure}
\caption{Sparse logistic regression: performance on large scale datasets, using $\lambda = 0.01\lambda_{\max}$.
	On the $x$-axis is the number of matrix-vector products computed,
	on the $y$-axis is the relative error $\|x^k-x^\star\|_{\infty}/\|x^\star\|_{\infty}$.
%	In \Cref{alg:zerofpr} we used L-BFGS directions.
}%
	\label{fig:SparseLogReg2}
\end{figure}


==> TeX/Tikz/DictLearning/matfact_perf_objvalue.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
% width=6.028in,
% height=4.754in,
grid,
at={(1.011in,0.642in)},
scale only axis,
xmin=0.98,
xmax=1.5,
ymin=0,
ymax=1,
axis background/.style={fill=white},
title style={font=\bfseries},
title={objective value performance},
legend style={legend cell align=left,align=left,draw=white!15!black},
legend pos=south east
]
\addplot [color=color_FBS,solid,line width=2.0pt,mark size=2.0pt,mark=x,mark options={solid}]
  table[row sep=crcr]{%
1	0.02\\
1	0.02\\
1	0.04\\
1	0.04\\
1	0.06\\
1	0.06\\
1	0.08\\
1	0.08\\
1	0.1\\
1	0.1\\
1	0.12\\
1	0.12\\
1	0.14\\
1	0.14\\
1	0.16\\
1	0.16\\
1	0.18\\
1	0.18\\
1	0.2\\
1	0.2\\
1	0.22\\
1	0.22\\
1	0.24\\
1	0.24\\
1	0.26\\
1	0.26\\
1	0.28\\
1	0.28\\
1	0.3\\
1	0.3\\
1	0.32\\
1	0.32\\
1	0.34\\
1	0.34\\
1	0.36\\
1	0.36\\
1	0.38\\
1	0.38\\
1	0.4\\
1	0.4\\
1	0.42\\
1	0.42\\
1	0.44\\
1	0.44\\
1	0.46\\
1	0.46\\
1	0.48\\
1	0.48\\
1	0.5\\
1	0.5\\
1	0.52\\
1	0.52\\
1	0.54\\
1	0.54\\
1	0.56\\
1	0.56\\
1	0.58\\
1	0.58\\
1	0.6\\
1	0.6\\
1	0.62\\
1	0.62\\
1	0.64\\
1	0.64\\
1	0.66\\
1	0.66\\
1	0.68\\
1	0.68\\
1	0.7\\
1	0.7\\
1	0.72\\
1.00037492450737	0.72\\
1.00037492450737	0.74\\
1.00591269792166	0.74\\
1.00591269792166	0.76\\
1.00681017958435	0.76\\
1.00681017958435	0.78\\
1.00878454770437	0.78\\
1.00878454770437	0.8\\
1.01144675980766	0.8\\
1.01144675980766	0.82\\
1.01856645353837	0.82\\
1.01856645353837	0.84\\
1.0299066441227	0.84\\
1.0299066441227	0.86\\
1.034311776879	0.86\\
1.034311776879	0.88\\
1.03476486168594	0.88\\
1.03476486168594	0.9\\
1.04889929479286	0.9\\
1.04889929479286	0.92\\
1.05716273347569	0.92\\
1.05716273347569	0.94\\
1.05887597609684	0.94\\
1.05887597609684	0.96\\
1.05943735177656	0.96\\
1.05943735177656	0.98\\
1.08095692371553	0.98\\
1.08095692371553	1\\
};
\addlegendentry{FBS};

\addplot [color=color_BFGS,\linestylelimited,line width=2.0pt,mark size=2.0pt,mark=asterisk,mark options={solid}]
  table[row sep=crcr]{%
1	0.02\\
1	0.02\\
1	0.04\\
1	0.04\\
1	0.06\\
1	0.06\\
1	0.08\\
1	0.08\\
1	0.1\\
1	0.1\\
1	0.12\\
1	0.12\\
1	0.14\\
1	0.14\\
1	0.16\\
1	0.16\\
1	0.18\\
1	0.18\\
1	0.2\\
1	0.2\\
1	0.22\\
1	0.22\\
1	0.24\\
1	0.24\\
1	0.26\\
1	0.26\\
1	0.28\\
1.00075924033327	0.28\\
1.00075924033327	0.3\\
1.00348429119358	0.3\\
1.00348429119358	0.32\\
1.00432656326888	0.32\\
1.00432656326888	0.34\\
1.00458910165649	0.34\\
1.00458910165649	0.36\\
1.00508146003214	0.36\\
1.00508146003214	0.38\\
1.01207068620642	0.38\\
1.01207068620642	0.4\\
1.01258271021499	0.4\\
1.01258271021499	0.42\\
1.01717303657281	0.42\\
1.01717303657281	0.44\\
1.02038649039594	0.44\\
1.02038649039594	0.46\\
1.02162512312802	0.46\\
1.02162512312802	0.48\\
1.02330821832315	0.48\\
1.02330821832315	0.5\\
1.02336697882763	0.5\\
1.02336697882763	0.52\\
1.02822301585822	0.52\\
1.02822301585822	0.54\\
1.03095154918332	0.54\\
1.03095154918332	0.56\\
1.03219539021334	0.56\\
1.03219539021334	0.58\\
1.0391436574345	0.58\\
1.0391436574345	0.6\\
1.04042466882347	0.6\\
1.04042466882347	0.62\\
1.04063482214716	0.62\\
1.04063482214716	0.64\\
1.04272376495629	0.64\\
1.04272376495629	0.66\\
1.04485960887991	0.66\\
1.04485960887991	0.68\\
1.04545728293023	0.68\\
1.04545728293023	0.7\\
1.04799542296846	0.7\\
1.04799542296846	0.72\\
1.04845783921957	0.72\\
1.04845783921957	0.74\\
1.04950425977091	0.74\\
1.04950425977091	0.76\\
1.05402243192445	0.76\\
1.05402243192445	0.78\\
1.05644244570699	0.78\\
1.05644244570699	0.8\\
1.05837889509069	0.8\\
1.05837889509069	0.82\\
1.07258558949903	0.82\\
1.07258558949903	0.84\\
1.07341541495287	0.84\\
1.07341541495287	0.86\\
1.0802660762549	0.86\\
1.0802660762549	0.88\\
1.0910063872983	0.88\\
1.0910063872983	0.9\\
1.09369892257162	0.9\\
1.09369892257162	0.92\\
1.12161372218765	0.92\\
1.12161372218765	0.94\\
1.12488395049513	0.94\\
1.12488395049513	0.96\\
1.12901247341664	0.96\\
1.12901247341664	0.98\\
1.18793205063676	0.98\\
1.18793205063676	1\\
};
\addlegendentry{ZeroFPR(L-BFGS)};

\end{axis}
\end{tikzpicture}%


==> TeX/Tikz/DictLearning/old/matfact_perf_cputime.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
% width=6.028in,
% height=4.754in,
at={(1.011in,0.642in)},
grid,
scale only axis,
xmin=0,
xmax=50,
ymin=0,
ymax=1,
ylabel={Frequency},
xlabel={Performance ratio},
axis background/.style={fill=white},
title style={font=\bfseries},
title={CPU time},
legend style={legend cell align=left,align=left,draw=white!15!black},
legend pos=south east
]
\addplot [color=color_FBS,solid,mark size=1.5pt,mark=x,mark options={solid}]
  table[row sep=crcr]{%
7.12056939545666	0.0333333333333333\\
8.44473199928661	0.0333333333333333\\
8.44473199928661	0.0666666666666667\\
9.1739251911459	0.0666666666666667\\
9.1739251911459	0.1\\
10.6589112202642	0.1\\
10.6589112202642	0.133333333333333\\
11.8474948747537	0.133333333333333\\
11.8474948747537	0.166666666666667\\
12.331426967884	0.166666666666667\\
12.331426967884	0.2\\
12.7428387944249	0.2\\
12.7428387944249	0.233333333333333\\
15.6630538582773	0.233333333333333\\
15.6630538582773	0.266666666666667\\
16.3217979491954	0.266666666666667\\
16.3217979491954	0.3\\
18.128725014158	0.3\\
18.128725014158	0.333333333333333\\
18.7260403395639	0.333333333333333\\
18.7260403395639	0.366666666666667\\
19.596799141109	0.366666666666667\\
19.596799141109	0.4\\
19.628798569359	0.4\\
19.628798569359	0.433333333333333\\
19.9903403286624	0.433333333333333\\
19.9903403286624	0.466666666666667\\
20.731561581423	0.466666666666667\\
20.731561581423	0.5\\
22.1340863096676	0.5\\
22.1340863096676	0.533333333333333\\
22.2153457191578	0.533333333333333\\
22.2153457191578	0.566666666666667\\
23.7961022754328	0.566666666666667\\
23.7961022754328	0.6\\
26.4179110703534	0.6\\
26.4179110703534	0.633333333333333\\
26.6612204160457	0.633333333333333\\
26.6612204160457	0.666666666666667\\
26.7508731297321	0.666666666666667\\
26.7508731297321	0.7\\
27.0280849977658	0.7\\
27.0280849977658	0.733333333333333\\
29.6092317430543	0.733333333333333\\
29.6092317430543	0.766666666666667\\
39.4293723693619	0.766666666666667\\
39.4293723693619	0.8\\
46.4588142310473	0.8\\
46.4588142310473	0.833333333333333\\
48.7484264478174	0.833333333333333\\
48.7484264478174	0.866666666666667\\
52.5355084255515	0.866666666666667\\
52.5355084255515	0.9\\
55.0314558241265	0.9\\
55.0314558241265	0.933333333333333\\
56.8379167344782	0.933333333333333\\
56.8379167344782	0.966666666666667\\
70.7965025669505	0.966666666666667\\
70.7965025669505	1\\
};
\addlegendentry{FBS};

\addplot [color=color_AFBS,solid,mark size=1.5pt,mark=asterisk,mark options={solid}]
  table[row sep=crcr]{%
3.52761612354909	0.0333333333333333\\
3.68037243429687	0.0333333333333333\\
3.68037243429687	0.0666666666666667\\
3.86104682421084	0.0666666666666667\\
3.86104682421084	0.1\\
3.94037681790444	0.1\\
3.94037681790444	0.133333333333333\\
3.9727561473561	0.133333333333333\\
3.9727561473561	0.166666666666667\\
4.16485119146735	0.166666666666667\\
4.16485119146735	0.2\\
4.30404791255711	0.2\\
4.30404791255711	0.233333333333333\\
4.34684726125435	0.233333333333333\\
4.34684726125435	0.266666666666667\\
4.42147763906833	0.266666666666667\\
4.42147763906833	0.3\\
4.50365974051097	0.3\\
4.50365974051097	0.333333333333333\\
4.69693100772239	0.333333333333333\\
4.69693100772239	0.366666666666667\\
4.80065169689241	0.366666666666667\\
4.80065169689241	0.4\\
4.84398039489725	0.4\\
4.84398039489725	0.433333333333333\\
5.06019134338478	0.433333333333333\\
5.06019134338478	0.466666666666667\\
5.21140064846729	0.466666666666667\\
5.21140064846729	0.5\\
5.38262950754201	0.5\\
5.38262950754201	0.533333333333333\\
5.70014114872307	0.533333333333333\\
5.70014114872307	0.566666666666667\\
5.74753130806757	0.566666666666667\\
5.74753130806757	0.6\\
5.81244029319408	0.6\\
5.81244029319408	0.633333333333333\\
5.92970283208378	0.633333333333333\\
5.92970283208378	0.666666666666667\\
5.95659216128634	0.666666666666667\\
5.95659216128634	0.7\\
6.13506580168108	0.7\\
6.13506580168108	0.733333333333333\\
6.19603774311648	0.733333333333333\\
6.19603774311648	0.766666666666667\\
7.60323436775336	0.766666666666667\\
7.60323436775336	0.8\\
7.83199309107032	0.8\\
7.83199309107032	0.833333333333333\\
8.14834954213224	0.833333333333333\\
8.14834954213224	0.866666666666667\\
8.38048994587149	0.866666666666667\\
8.38048994587149	0.9\\
8.45325971678298	0.9\\
8.45325971678298	0.933333333333333\\
16.5505220297663	0.933333333333333\\
16.5505220297663	0.966666666666667\\
20.7839381203312	0.966666666666667\\
20.7839381203312	1\\
};
\addlegendentry{AFBS};

\addplot [color=color_BFGS,\linestylelimited,mark size=1.1pt,mark=square,mark options={solid}]
  table[row sep=crcr]{%
1	0.0333333333333333\\
1	0.0333333333333333\\
1	0.0666666666666667\\
1	0.0666666666666667\\
1	0.1\\
1	0.1\\
1	0.133333333333333\\
1	0.133333333333333\\
1	0.166666666666667\\
1	0.166666666666667\\
1	0.2\\
1	0.2\\
1	0.233333333333333\\
1	0.233333333333333\\
1	0.266666666666667\\
1	0.266666666666667\\
1	0.3\\
1	0.3\\
1	0.333333333333333\\
1	0.333333333333333\\
1	0.366666666666667\\
1	0.366666666666667\\
1	0.4\\
1	0.4\\
1	0.433333333333333\\
1	0.433333333333333\\
1	0.466666666666667\\
1	0.466666666666667\\
1	0.5\\
1	0.5\\
1	0.533333333333333\\
1	0.533333333333333\\
1	0.566666666666667\\
1	0.566666666666667\\
1	0.6\\
1	0.6\\
1	0.633333333333333\\
1	0.633333333333333\\
1	0.666666666666667\\
1	0.666666666666667\\
1	0.7\\
1	0.7\\
1	0.733333333333333\\
1	0.733333333333333\\
1	0.766666666666667\\
1	0.766666666666667\\
1	0.8\\
1	0.8\\
1	0.833333333333333\\
1	0.833333333333333\\
1	0.866666666666667\\
1	0.866666666666667\\
1	0.9\\
1	0.9\\
1	0.933333333333333\\
1	0.933333333333333\\
1	0.966666666666667\\
1	0.966666666666667\\
1	1\\
};
\addlegendentry{ZeroFPR(L-BFGS)};

\end{axis}
\end{tikzpicture}%


==> TeX/Tikz/DictLearning/old/matfact_perf_objvalue.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
% width=6.028in,
% height=4.754in,
at={(1.011in,0.642in)},
grid,
scale only axis,
xmin=0.98,
xmax=1.5,
ymin=0,
ymax=1,
ylabel={Frequency},
xlabel={Performance ratio},
axis background/.style={fill=white},
title style={font=\bfseries},
title={Final cost value},
legend style={legend cell align=left,align=left,draw=white!15!black},
legend pos=south east
]
\addplot [color=color_FBS,solid,mark size=1.5pt,mark=x,mark options={solid}]
  table[row sep=crcr]{%
1	0.0333333333333333\\
1	0.0333333333333333\\
1	0.0666666666666667\\
1	0.0666666666666667\\
1	0.1\\
1	0.1\\
1	0.133333333333333\\
1	0.133333333333333\\
1	0.166666666666667\\
1.00804189810215	0.166666666666667\\
1.00804189810215	0.2\\
1.00906439242663	0.2\\
1.00906439242663	0.233333333333333\\
1.01108942703187	0.233333333333333\\
1.01108942703187	0.266666666666667\\
1.0156015829267	0.266666666666667\\
1.0156015829267	0.3\\
1.03131168366742	0.3\\
1.03131168366742	0.333333333333333\\
1.03221025914165	0.333333333333333\\
1.03221025914165	0.366666666666667\\
1.03470967079588	0.366666666666667\\
1.03470967079588	0.4\\
1.03693176298359	0.4\\
1.03693176298359	0.433333333333333\\
1.03817739307334	0.433333333333333\\
1.03817739307334	0.466666666666667\\
1.04101606998572	0.466666666666667\\
1.04101606998572	0.5\\
1.0454225815928	0.5\\
1.0454225815928	0.533333333333333\\
1.04552927924348	0.533333333333333\\
1.04552927924348	0.566666666666667\\
1.04832591701796	0.566666666666667\\
1.04832591701796	0.6\\
1.04915633974541	0.6\\
1.04915633974541	0.633333333333333\\
1.05402904672976	0.633333333333333\\
1.05402904672976	0.666666666666667\\
1.05853663520271	0.666666666666667\\
1.05853663520271	0.7\\
1.06335091187807	0.7\\
1.06335091187807	0.733333333333333\\
1.06589562901738	0.733333333333333\\
1.06589562901738	0.766666666666667\\
1.06665528983726	0.766666666666667\\
1.06665528983726	0.8\\
1.06809010617115	0.8\\
1.06809010617115	0.833333333333333\\
1.06989096099067	0.833333333333333\\
1.06989096099067	0.866666666666667\\
1.07237788754816	0.866666666666667\\
1.07237788754816	0.9\\
1.07786258053514	0.9\\
1.07786258053514	0.933333333333333\\
1.0855721941926	0.933333333333333\\
1.0855721941926	0.966666666666667\\
1.09119776386213	0.966666666666667\\
1.09119776386213	1\\
};
\addlegendentry{FBS};

\addplot [color=color_AFBS,solid,mark size=1.5pt,mark=asterisk,mark options={solid}]
  table[row sep=crcr]{%
1	0.0333333333333333\\
1	0.0333333333333333\\
1	0.0666666666666667\\
1	0.0666666666666667\\
1	0.1\\
1	0.1\\
1	0.133333333333333\\
1	0.133333333333333\\
1	0.166666666666667\\
1	0.166666666666667\\
1	0.2\\
1	0.2\\
1	0.233333333333333\\
1	0.233333333333333\\
1	0.266666666666667\\
1	0.266666666666667\\
1	0.3\\
1	0.3\\
1	0.333333333333333\\
1	0.333333333333333\\
1	0.366666666666667\\
1	0.366666666666667\\
1	0.4\\
1	0.4\\
1	0.433333333333333\\
1	0.433333333333333\\
1	0.466666666666667\\
1	0.466666666666667\\
1	0.5\\
1	0.5\\
1	0.533333333333333\\
1	0.533333333333333\\
1	0.566666666666667\\
1	0.566666666666667\\
1	0.6\\
1	0.6\\
1	0.633333333333333\\
1	0.633333333333333\\
1	0.666666666666667\\
1	0.666666666666667\\
1	0.7\\
1	0.7\\
1	0.733333333333333\\
1	0.733333333333333\\
1	0.766666666666667\\
1	0.766666666666667\\
1	0.8\\
1.01592657831818	0.8\\
1.01592657831818	0.833333333333333\\
1.02151612086907	0.833333333333333\\
1.02151612086907	0.866666666666667\\
1.02865871319276	0.866666666666667\\
1.02865871319276	0.9\\
1.06188387629936	0.9\\
1.06188387629936	0.933333333333333\\
1.06328318844248	0.933333333333333\\
1.06328318844248	0.966666666666667\\
1.06634060818787	0.966666666666667\\
1.06634060818787	1\\
};
\addlegendentry{AFBS};

\addplot [color=color_BFGS,\linestylelimited,mark size=1.1pt,mark=square,mark options={solid}]
  table[row sep=crcr]{%
1	0.0333333333333333\\
1.00694908506859	0.0333333333333333\\
1.00694908506859	0.0666666666666667\\
1.02024086754245	0.0666666666666667\\
1.02024086754245	0.1\\
1.02284686642868	0.1\\
1.02284686642868	0.133333333333333\\
1.02517527003238	0.133333333333333\\
1.02517527003238	0.166666666666667\\
1.03114073601117	0.166666666666667\\
1.03114073601117	0.2\\
1.03461055599974	0.2\\
1.03461055599974	0.233333333333333\\
1.03591701084029	0.233333333333333\\
1.03591701084029	0.266666666666667\\
1.04528977308572	0.266666666666667\\
1.04528977308572	0.3\\
1.04556086438295	0.3\\
1.04556086438295	0.333333333333333\\
1.04852497299148	0.333333333333333\\
1.04852497299148	0.366666666666667\\
1.0497425972053	0.366666666666667\\
1.0497425972053	0.4\\
1.05388518858308	0.4\\
1.05388518858308	0.433333333333333\\
1.05406658651375	0.433333333333333\\
1.05406658651375	0.466666666666667\\
1.05426182953963	0.466666666666667\\
1.05426182953963	0.5\\
1.06344002951397	0.5\\
1.06344002951397	0.533333333333333\\
1.0644718838888	0.533333333333333\\
1.0644718838888	0.566666666666667\\
1.06704242238623	0.566666666666667\\
1.06704242238623	0.6\\
1.06905853469947	0.6\\
1.06905853469947	0.633333333333333\\
1.07223690413305	0.633333333333333\\
1.07223690413305	0.666666666666667\\
1.07667965998388	0.666666666666667\\
1.07667965998388	0.7\\
1.07777520853132	0.7\\
1.07777520853132	0.733333333333333\\
1.08192581029001	0.733333333333333\\
1.08192581029001	0.766666666666667\\
1.09086441163597	0.766666666666667\\
1.09086441163597	0.8\\
1.09098308984294	0.8\\
1.09098308984294	0.833333333333333\\
1.09307984798761	0.833333333333333\\
1.09307984798761	0.866666666666667\\
1.09703805711482	0.866666666666667\\
1.09703805711482	0.9\\
1.12838346714899	0.9\\
1.12838346714899	0.933333333333333\\
1.12840679452564	0.933333333333333\\
1.12840679452564	0.966666666666667\\
1.14082202335722	0.966666666666667\\
1.14082202335722	1\\
};
\addlegendentry{ZeroFPR(L-BFGS)};

\end{axis}
\end{tikzpicture}%


==> TeX/Tikz/MatComp/MatComp_10.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}

\begin{axis}[%
% width=4.521in,
% height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=200,
ymin=0,
ymax=400000,
axis background/.style={fill=white},
legend style={legend cell align=left,align=left,draw=white!15!black}
]
\addplot [color=mycolor1,solid,line width=1.5pt]
  table[row sep=crcr]{%
1	365502.499238357\\
2	204209.725153528\\
3	146754.001900892\\
4	117069.323327051\\
5	98993.0479201509\\
6	86857.7390532334\\
7	78160.0112931126\\
8	71626.0361436578\\
9	66540.6622976267\\
10	62471.9339696853\\
11	59143.7353284282\\
12	56371.4064976994\\
13	54026.8155002005\\
14	52018.2922029479\\
15	50278.5391439245\\
16	48757.0505351405\\
17	47415.1930715385\\
18	46222.9185559633\\
19	45156.510035414\\
20	44197.0014219025\\
21	43329.0471308422\\
22	42540.0991738931\\
23	41819.7985090532\\
24	41159.518377616\\
25	40552.0171970619\\
26	39991.1715807285\\
27	39471.7687422203\\
28	38989.343449742\\
29	38540.0487773158\\
30	38120.5527619716\\
31	37727.9551100538\\
32	37359.7195595104\\
33	37013.618570384\\
34	36687.6877995359\\
35	36380.1883980281\\
36	36089.5756063513\\
37	35814.4724531693\\
38	35553.6476153056\\
39	35305.9966904987\\
40	35070.5262845339\\
41	34846.3404314033\\
42	34632.6289570424\\
43	34428.6574697936\\
44	34233.7587184618\\
45	34047.3251049605\\
46	33868.8021756387\\
47	33697.6829453565\\
48	33533.502932703\\
49	33375.8358046473\\
50	33224.2895451624\\
51	33078.5030758024\\
52	32938.1432672866\\
53	32802.9022903557\\
54	32672.4952618328\\
55	32546.6581482409\\
56	32425.1458947113\\
57	32307.7307514573\\
58	32194.2007739094\\
59	32084.3584758645\\
60	31978.0196177521\\
61	31875.0121144846\\
62	31775.1750493493\\
63	31678.3577821443\\
64	31584.4191412226\\
65	31493.2266903935\\
66	31404.6560627261\\
67	31318.5903542517\\
68	31234.9195713894\\
69	31153.5401266359\\
70	31074.3543776846\\
71	30997.2702056863\\
72	30922.2006288382\\
73	30849.06344791\\
74	30777.7809206793\\
75	30708.2794625732\\
76	30640.4893710977\\
77	30574.3445718869\\
78	30509.7823844256\\
79	30446.7433057014\\
80	30385.1708102059\\
81	30325.0111648723\\
82	30266.2132576663\\
83	30208.7284386747\\
84	30152.5103726446\\
85	30097.5149020258\\
86	30043.6999196552\\
87	29991.0252503028\\
88	29939.4525403701\\
89	29888.9451550942\\
90	29839.4680826693\\
91	29790.9878447487\\
92	29743.4724128382\\
93	29696.8911301321\\
94	29651.2146383844\\
95	29606.4148094385\\
96	29562.4646810705\\
97	29519.3383968402\\
98	29477.0111496466\\
99	29435.4591287357\\
100	29394.6594699075\\
101	29354.5902087037\\
102	29315.2302363647\\
103	29276.5592583687\\
104	29238.5577553759\\
105	29201.2069464152\\
106	29164.4887541644\\
107	29128.3857721851\\
108	29092.8812339838\\
109	29057.9589837816\\
110	29023.603448882\\
111	28989.7996135347\\
112	28956.532994204\\
113	28923.7896161459\\
114	28891.5559912246\\
115	28859.8190968824\\
116	28828.5663561983\\
117	28797.785618967\\
118	28767.4651437393\\
119	28737.5935807648\\
120	28708.1599557875\\
121	28679.15365464\\
122	28650.5644085947\\
123	28622.3822804259\\
124	28594.5976511433\\
125	28567.2012073605\\
126	28540.1839292609\\
127	28513.5370791297\\
128	28487.2521904205\\
129	28461.3210573271\\
130	28435.7357248354\\
131	28410.4884792243\\
132	28385.5718390004\\
133	28360.9785462324\\
134	28336.7015582799\\
135	28312.7340398792\\
136	28289.0693555785\\
137	28265.7010625026\\
138	28242.6229034291\\
139	28219.8288001611\\
140	28197.3128471818\\
141	28175.0693055774\\
142	28153.0925972142\\
143	28131.3772991577\\
144	28109.9181383235\\
145	28088.709986347\\
146	28067.7478546619\\
147	28047.0268897789\\
148	28026.5423687529\\
149	28006.2896948317\\
150	27986.2643932794\\
151	27966.4621073609\\
152	27946.8785944851\\
153	27927.5097225009\\
154	27908.3514661297\\
155	27889.3999035409\\
156	27870.6512130561\\
157	27852.1016699782\\
158	27833.7476435395\\
159	27815.5855939631\\
160	27797.6120696373\\
161	27779.8237043904\\
162	27762.2172148676\\
163	27744.7893980036\\
164	27727.5371285861\\
165	27710.4573569085\\
166	27693.5471065055\\
167	27676.8034719702\\
168	27660.2236168485\\
169	27643.8047716071\\
170	27627.5442316721\\
171	27611.4393555418\\
172	27595.4875629527\\
173	27579.6863331191\\
174	27564.0332030339\\
175	27548.5257658153\\
176	27533.1616691214\\
177	27517.9386136147\\
178	27502.8543514735\\
179	27487.9066849637\\
180	27473.0934650414\\
181	27458.4125900164\\
182	27443.8620042527\\
183	27429.4396969126\\
184	27415.1437007405\\
185	27400.9720908874\\
186	27386.9229837716\\
187	27372.9945359769\\
188	27359.1849431855\\
189	27345.4924391424\\
190	27331.9152946562\\
191	27318.451816629\\
192	27305.100347112\\
193	27291.8592624015\\
194	27278.7269721515\\
195	27265.7019185179\\
196	27252.7825753297\\
197	27239.9674472825\\
198	27227.2550691611\\
199	27214.6440050771\\
200	27202.1328477391\\
};
\addlegendentry{fbs,basic,none,none};

\addplot [color=mycolor2,solid,line width=1.5pt]
  table[row sep=crcr]{%
1	381544.974276441\\
3	152833.821583277\\
5	84363.2968186438\\
7	65266.7360348166\\
9	53538.0669934081\\
11	46873.7087232143\\
13	42318.1279382231\\
15	39231.6677332606\\
17	36898.5623241272\\
19	35287.8668204404\\
21	33961.2042470137\\
23	32951.6913059661\\
25	32128.2675848752\\
27	31462.8938805877\\
29	30889.9366633073\\
31	30420.5677311678\\
33	30006.8528113695\\
35	29648.9730066532\\
37	29333.2135159772\\
39	29056.5959178042\\
41	28805.0137119803\\
43	28581.749255635\\
45	28378.5562824595\\
47	28193.0196886432\\
49	28022.0370015413\\
51	27865.5706447303\\
53	27719.1683782668\\
55	27583.0290387352\\
57	27455.8143067426\\
59	27336.377102031\\
61	27223.3988079735\\
63	27117.2558424217\\
65	27016.6745111804\\
67	26921.2060438389\\
69	26830.6575772972\\
71	26744.7349899892\\
73	26662.6832208545\\
75	26584.5541099574\\
77	26510.0772437769\\
79	26438.8675668541\\
81	26370.7643111299\\
83	26305.7786780388\\
85	26243.572702956\\
87	26184.0081963764\\
89	26127.0314378602\\
91	26072.4346974256\\
93	26019.9742309775\\
95	25969.5883376383\\
97	25921.1089983873\\
99	25874.3393875536\\
101	25829.2052235344\\
103	25785.6534024823\\
105	25743.5577281677\\
107	25702.8822573864\\
109	25663.6231261587\\
111	25625.712369077\\
113	25589.0903499053\\
115	25553.740464352\\
117	25519.5890159824\\
119	25486.5446072282\\
121	25454.5535516846\\
123	25423.5492450103\\
125	25393.4417049001\\
127	25364.1806869443\\
129	25335.730557838\\
131	25308.0398846099\\
133	25281.0784607721\\
135	25254.8396977618\\
137	25229.3004606391\\
139	25204.4382791573\\
141	25180.2471888365\\
143	25156.7098163497\\
145	25133.7966714507\\
147	25111.4895790664\\
149	25089.7677315142\\
151	25068.5980376106\\
153	25047.9539621251\\
155	25027.8147300544\\
157	25008.1512382312\\
159	24988.9370236169\\
161	24970.1547988407\\
163	24951.784475342\\
165	24933.8054153208\\
167	24916.206062175\\
169	24898.9762810257\\
171	24882.1035172569\\
173	24865.5808629313\\
175	24849.4044248355\\
177	24833.5663891787\\
179	24818.0598791329\\
181	24802.8804115149\\
183	24788.0195928875\\
185	24773.466740724\\
187	24759.2130112796\\
189	24745.2476165828\\
191	24731.5570603207\\
193	24718.1296564759\\
195	24704.9544657124\\
197	24692.0189723231\\
199	24679.3123049794\\
};
\addlegendentry{zerofpr,,lbroyden,backtracking-nm};

\addplot [color=mycolor3,solid,line width=1.5pt]
  table[row sep=crcr]{%
1	381544.97427643\\
3	152833.821583293\\
5	84363.2968186828\\
7	65333.6993051992\\
9	53042.5569557797\\
11	46406.4885506068\\
13	44502.8969899885\\
15	37161.134001836\\
17	34438.5129136003\\
19	33298.2661827731\\
21	32217.1039644292\\
23	31965.8905372478\\
25	30620.3247484521\\
27	30220.4331534732\\
29	29862.8891719015\\
31	29334.5553301506\\
33	29224.1500332548\\
35	28660.0142490236\\
37	28544.3135133388\\
39	28383.8527232495\\
41	28128.901073446\\
43	28072.1940143859\\
45	27730.1287117166\\
47	27654.792797286\\
49	27545.1567712273\\
51	27358.2321544494\\
53	27317.9206473426\\
55	27089.141933825\\
57	27043.6586555657\\
59	26968.6475816903\\
61	26838.3373679251\\
63	26810.335244118\\
65	26637.9737941153\\
67	26601.2500036537\\
69	26542.1046374939\\
71	26440.2065523223\\
73	26417.3379631753\\
75	26284.3219190609\\
77	26258.1020999705\\
79	26212.5707171398\\
81	26131.4130937246\\
83	26113.9598354\\
85	26005.4503229066\\
87	25982.6004058126\\
89	25944.3870633509\\
91	25878.1237476354\\
93	25863.0328676581\\
95	25774.4148706438\\
97	25757.0120296773\\
99	25726.1952694045\\
101	25670.6984629701\\
103	25658.6585655797\\
105	25583.2538427041\\
107	25567.4626974974\\
109	25540.5244536654\\
111	25493.5264501489\\
113	25482.7423934864\\
115	25419.0098645427\\
117	25406.5082700842\\
119	25384.1412719295\\
121	25343.5795236304\\
123	25334.7117009999\\
125	25278.8447310873\\
127	25267.1748352097\\
129	25247.0163528274\\
131	25211.6419419484\\
133	25203.486560307\\
135	25155.0503859868\\
137	25145.5474219911\\
139	25128.4285729288\\
141	25097.216177834\\
143	25090.3521962836\\
145	25046.9185061132\\
147	25037.8519126845\\
149	25022.0554399114\\
151	24994.2029115544\\
153	24987.7591358714\\
155	24949.3543458324\\
157	24941.8116154627\\
159	24928.1559540925\\
161	24903.1553886053\\
163	24897.6334987924\\
165	24862.591667616\\
167	24855.2742240956\\
169	24842.4463829491\\
171	24819.7454333852\\
173	24814.4798904616\\
175	24783.0313594834\\
177	24776.8458427822\\
179	24765.606088943\\
181	24744.9675614258\\
183	24740.3941834115\\
185	24711.3261380564\\
187	24705.2512318372\\
189	24694.5534310204\\
191	24675.5702433021\\
193	24671.1587256127\\
195	24644.7841620039\\
197	24639.5883698117\\
199	24630.1213711483\\
};
\addlegendentry{zerofpr,,rbroyden,backtracking-nm};

\addplot [color=mycolor4,solid,line width=1.5pt]
  table[row sep=crcr]{%
1	381544.974276444\\
3	152833.821583288\\
5	71369.6447545433\\
7	50930.4678804912\\
9	40624.5075298759\\
11	36510.8808329002\\
13	33547.2489344442\\
15	31992.8347588955\\
17	30841.2575068369\\
19	30025.6849843545\\
21	29449.342566113\\
23	28855.7373241891\\
25	28465.7556107916\\
27	28143.6564949141\\
29	27848.6326584813\\
31	27586.5950189366\\
33	27375.1533843803\\
35	27178.0158658406\\
37	27008.9028191561\\
39	26836.169389781\\
41	26680.3103299026\\
43	26553.8191016603\\
45	26437.0543909739\\
47	26301.2727666956\\
49	26173.846047958\\
51	26063.6965892009\\
53	25976.843755826\\
55	25875.9443438604\\
57	25787.7489939767\\
59	25695.6819256009\\
61	25626.8612318566\\
63	25546.8945041455\\
65	25479.3120487329\\
67	25406.458860245\\
69	25351.0893401376\\
71	25287.4152065343\\
73	25233.0700062807\\
75	25172.6662622474\\
77	25124.4836252165\\
79	25074.6965120883\\
81	25032.184284053\\
83	24983.3334786248\\
85	24942.5310066058\\
87	24900.2054976204\\
89	24863.7081505334\\
91	24822.3460990483\\
93	24787.1650436004\\
95	24750.5894779582\\
97	24719.9248138246\\
99	24685.8992568337\\
101	24656.7715082192\\
103	24625.7325741862\\
105	24599.2660250583\\
107	24571.4214380486\\
109	24546.5199346098\\
111	24519.0889910591\\
113	24494.7578448311\\
115	24469.6481128518\\
117	24447.3569438889\\
119	24423.9347721533\\
121	24402.7894067814\\
123	24380.7535053033\\
125	24360.8043265439\\
127	24340.0267368268\\
129	24320.9391540597\\
131	24301.1280144481\\
133	24283.0199895973\\
135	24264.4809474434\\
137	24247.5447079113\\
139	24229.9570311285\\
141	24213.746367842\\
143	24196.7674750099\\
145	24181.0285376981\\
147	24164.7861962827\\
149	24149.9201021566\\
151	24134.7082952843\\
153	24120.5552948695\\
155	24105.569563219\\
157	24091.3353803641\\
159	24076.3044614077\\
161	24062.3631158293\\
163	24048.0038254068\\
165	24034.7355230447\\
167	24020.858428103\\
169	24008.0101663577\\
171	23994.5794079466\\
173	23982.2686680884\\
175	23969.4211567225\\
177	23957.5374356522\\
179	23945.1537369373\\
181	23933.7452065721\\
183	23921.972926174\\
185	23911.0140519367\\
187	23899.444071079\\
189	23888.5038947927\\
191	23877.003686123\\
193	23866.414705274\\
195	23855.5995916952\\
197	23845.759008043\\
199	23835.593206297\\
};
\addlegendentry{zerofpr,,lbfgs,backtracking-nm};

\end{axis}
\end{tikzpicture}%


==> TeX/Tikz/MatComp/MatComp_15.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
% \definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
% \definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
% \definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
% \definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}

\begin{axis}[%
% width=1.2in,
% height=1.0in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=200,
ymin=1e4,
ymax=1e5,
xmajorgrids,
ymajorgrids,
xlabel={number of SVDs},
ylabel={$\varphi(x^k)$},
axis background/.style={fill=white},
legend style={legend cell align=left,align=left,draw=white!15!black}
]
\addplot [color=color_FBS,line width=1.5pt]
  table[row sep=crcr]{%
1	345643.766883559\\
2	188106.430182279\\
3	133726.324760836\\
4	105994.656745639\\
5	89229.7899455682\\
6	78024.5088163696\\
7	70015.4140266714\\
8	64008.5117407244\\
9	59337.0577294452\\
10	55600.0893335219\\
11	52542.2649304407\\
12	49993.3834635826\\
13	47835.688813385\\
14	45985.1439076431\\
15	44380.1819184923\\
16	42974.6728169889\\
17	41733.3728937703\\
18	40628.8926669113\\
19	39639.6239111451\\
20	38748.2899516984\\
21	37940.9112293621\\
22	37206.0537799531\\
23	36534.2743390814\\
24	35917.7045816712\\
25	35349.7354341109\\
26	34824.7744412443\\
27	34338.0571946251\\
28	33885.499269057\\
29	33463.5788631414\\
30	33069.2429609531\\
31	32699.8316905871\\
32	32353.0168897653\\
33	32026.7518583095\\
34	31719.2299895983\\
35	31428.8505018039\\
36	31154.1898859094\\
37	30893.9779871198\\
38	30647.07786478\\
39	30412.4687515834\\
40	30189.2315689273\\
41	29976.5365614064\\
42	29773.6326968363\\
43	29579.8385440519\\
44	29394.5343931545\\
45	29217.1554247688\\
46	29047.1857685694\\
47	28884.1533185719\\
48	28727.6251947937\\
49	28577.2037589572\\
50	28432.5231066923\\
51	28293.2459708814\\
52	28159.0609808572\\
53	28029.6802305273\\
54	27904.8371154464\\
55	27784.2844046939\\
56	27667.7925182788\\
57	27555.147984917\\
58	27446.1520584894\\
59	27340.6194744296\\
60	27238.3773297899\\
61	27139.2640728615\\
62	27043.1285900425\\
63	26949.82937921\\
64	26859.2338001874\\
65	26771.2173940544\\
66	26685.6632640436\\
67	26602.4615116295\\
68	26521.5087221634\\
69	26442.7074950606\\
70	26365.9660141123\\
71	26291.1976539924\\
72	26218.3206194589\\
73	26147.2576141355\\
74	26077.9355360914\\
75	26010.28519773\\
76	25944.2410677616\\
77	25879.7410332596\\
78	25816.7261800078\\
79	25755.1405895245\\
80	25694.9311513091\\
81	25636.0473889999\\
82	25578.4412992612\\
83	25522.0672023261\\
84	25466.8816032271\\
85	25412.8430628372\\
86	25359.9120779212\\
87	25308.0509694752\\
88	25257.2237786956\\
89	25207.3961699751\\
90	25158.5353403828\\
91	25110.6099351261\\
92	25063.5899685407\\
93	25017.4467501924\\
94	24972.1528157082\\
95	24927.6818619891\\
96	24884.0086864834\\
97	24841.1091302277\\
98	24798.9600243855\\
99	24757.5391400359\\
100	24716.825140984\\
101	24676.7975393826\\
102	24637.4366539732\\
103	24598.7235707659\\
104	24560.6401059956\\
105	24523.1687712003\\
106	24486.2927402828\\
107	24449.9958184238\\
108	24414.2624127283\\
109	24379.0775044911\\
110	24344.4266229807\\
111	24310.2958206428\\
112	24276.6716496377\\
113	24243.541139625\\
114	24210.891776722\\
115	24178.7114835628\\
116	24146.9886003908\\
117	24115.7118671247\\
118	24084.8704063376\\
119	24054.4537070976\\
120	24024.4516096168\\
121	23994.8542906667\\
122	23965.6522497097\\
123	23936.8362957104\\
124	23908.3975345866\\
125	23880.3273572643\\
126	23852.617428303\\
127	23825.25967506\\
128	23798.2462773641\\
129	23771.5696576708\\
130	23745.2224716732\\
131	23719.1975993446\\
132	23693.4881363891\\
133	23668.0873860791\\
134	23642.9888514597\\
135	23618.1862279004\\
136	23593.6733959766\\
137	23569.4444146639\\
138	23545.4935148291\\
139	23521.8150930036\\
140	23498.4037054242\\
141	23475.2540623282\\
142	23452.3610224912\\
143	23429.7195879939\\
144	23407.324899209\\
145	23385.1722299948\\
146	23363.2569830887\\
147	23341.5746856882\\
148	23320.1209852125\\
149	23298.8916452352\\
150	23277.8825415802\\
151	23257.0896585739\\
152	23236.5090854453\\
153	23216.1370128682\\
154	23195.969729639\\
155	23176.0036194831\\
156	23156.2351579849\\
157	23136.6609096357\\
158	23117.2775249944\\
159	23098.0817379552\\
160	23079.0703631189\\
161	23060.2402932621\\
162	23041.5884969011\\
163	23023.1120159455\\
164	23004.8079634376\\
165	22986.673521376\\
166	22968.7059386163\\
167	22950.9025288485\\
168	22933.2606686477\\
169	22915.7777955925\\
170	22898.4514064524\\
171	22881.279055437\\
172	22864.2583525082\\
173	22847.3869617503\\
174	22830.6625997971\\
175	22814.083034313\\
176	22797.6460825259\\
177	22781.349609811\\
178	22765.1915283217\\
179	22749.1697956671\\
180	22733.2824136335\\
181	22717.5274269496\\
182	22701.9029220909\\
183	22686.4070261254\\
184	22671.037905596\\
185	22655.7937654398\\
186	22640.6728479427\\
187	22625.6734317274\\
188	22610.7938307743\\
189	22596.0323934737\\
190	22581.387501708\\
191	22566.8575699632\\
192	22552.4410444682\\
193	22538.1364023615\\
194	22523.9421508838\\
195	22509.856826595\\
196	22495.878994617\\
197	22482.0072478979\\
198	22468.2402065006\\
199	22454.5765169119\\
200	22441.014851373\\
};
\addlegendentry{FBS};

%\addplot [color=mycolor2,solid,line width=1.5pt]
%  table[row sep=crcr]{%
%1	362679.17853937\\
%3	139455.679423498\\
%5	76429.3745698591\\
%7	58732.5350769636\\
%9	47846.9636012395\\
%11	41623.611325828\\
%13	37309.1641662308\\
%15	34412.0263681786\\
%17	32158.8324083342\\
%19	30617.8822632953\\
%21	29346.2375632685\\
%23	28382.1497744552\\
%25	27588.2345642321\\
%27	26947.5982675989\\
%29	26387.1987454421\\
%31	25925.261600016\\
%33	25513.1371259944\\
%35	25153.3799819659\\
%37	24830.0360830565\\
%39	24543.3534474022\\
%41	24277.8588643847\\
%43	24039.1261838859\\
%45	23818.9629642559\\
%47	23616.4221954846\\
%49	23428.0384073138\\
%51	23254.7588694282\\
%53	23091.7338219198\\
%55	22939.5741365889\\
%57	22796.8298406923\\
%59	22662.6497929019\\
%61	22535.565622823\\
%63	22416.1326773823\\
%65	22302.9139691325\\
%67	22195.4233068471\\
%69	22093.2968420608\\
%71	21996.186898376\\
%73	21903.1938149352\\
%75	21814.3642288325\\
%77	21729.3905443223\\
%79	21647.910757047\\
%81	21569.7766357587\\
%83	21495.0556587369\\
%85	21423.4209392627\\
%87	21354.7709401636\\
%89	21289.0689026565\\
%91	21226.1193816332\\
%93	21165.6754672313\\
%95	21107.6789448462\\
%97	21051.9448172616\\
%99	20998.258613865\\
%101	20946.5211640754\\
%103	20896.6486937972\\
%105	20848.4784820927\\
%107	20801.9412130859\\
%109	20756.997155151\\
%111	20713.5479344214\\
%113	20671.510850695\\
%115	20630.8527579438\\
%117	20591.4900001528\\
%119	20553.3308895374\\
%121	20516.3263952233\\
%123	20480.4182344276\\
%125	20445.5290447926\\
%127	20411.6223990973\\
%129	20378.6741257761\\
%131	20346.6432951437\\
%133	20315.5074126066\\
%135	20285.2620454757\\
%137	20255.8825662036\\
%139	20227.3423469487\\
%141	20199.6269954224\\
%143	20172.7086826537\\
%145	20146.54793014\\
%147	20121.116184535\\
%149	20096.3828382237\\
%151	20072.3078685775\\
%153	20048.8598203339\\
%155	20026.0142334331\\
%157	20003.7407141257\\
%159	19982.0131422846\\
%161	19960.8144729686\\
%163	19940.1250731666\\
%165	19919.9248375157\\
%167	19900.2013049151\\
%169	19880.9420412568\\
%171	19862.1314531863\\
%173	19843.7581273879\\
%175	19825.8121786645\\
%177	19808.2793898434\\
%179	19791.146099759\\
%181	19774.400581159\\
%183	19758.0277469538\\
%185	19742.0112306745\\
%187	19726.3373205101\\
%189	19710.9916868893\\
%191	19695.9590190939\\
%193	19681.2271005742\\
%195	19666.7855520929\\
%197	19652.6235467559\\
%199	19638.7324358151\\
%};
%\addlegendentry{L-Broyden};
%
%\addplot [color=mycolor3,solid,line width=1.5pt]
%  table[row sep=crcr]{%
%1	362679.178539389\\
%3	139455.679423506\\
%5	76429.3745698614\\
%7	58768.5200406608\\
%9	47350.2486502143\\
%11	41175.3002531073\\
%13	39351.8765474442\\
%15	32610.0354965431\\
%17	29804.044371359\\
%19	28754.5841795707\\
%21	27687.3608540286\\
%23	27438.8561411674\\
%25	26106.8513369705\\
%27	25675.2324822085\\
%29	25307.541906069\\
%31	24728.4870006273\\
%33	24612.3872777271\\
%35	24040.7144742362\\
%37	23913.1537383632\\
%39	23746.14803318\\
%41	23495.9757820986\\
%43	23433.7034051317\\
%45	23067.2581794272\\
%47	22985.6933254543\\
%49	22863.2428307595\\
%51	22643.4739153358\\
%53	22599.3239980269\\
%55	22347.9963786965\\
%57	22295.4734246444\\
%59	22211.5893569209\\
%61	22069.1018258038\\
%63	22037.1219707693\\
%65	21848.0940332514\\
%67	21808.0188417362\\
%69	21742.8684387087\\
%71	21628.3079540481\\
%73	21603.1747323717\\
%75	21455.2278630053\\
%77	21424.9897341483\\
%79	21373.2589098787\\
%81	21281.8430064074\\
%83	21261.874963175\\
%85	21142.4091894965\\
%87	21117.4111130975\\
%89	21075.1671045305\\
%91	21000.4585717301\\
%93	20983.7680767069\\
%95	20884.3412509733\\
%97	20864.1081988067\\
%99	20828.5738664016\\
%101	20764.8078697001\\
%103	20750.8425722565\\
%105	20666.3620628212\\
%107	20648.7631127187\\
%109	20618.3032992534\\
%111	20563.9878005508\\
%113	20551.8003741974\\
%115	20478.7658918765\\
%117	20463.9086850595\\
%119	20437.4875740697\\
%121	20389.7419084065\\
%123	20379.2189462807\\
%125	20315.1335349967\\
%127	20301.815718634\\
%129	20278.4224497357\\
%131	20236.5133402802\\
%133	20227.0886223866\\
%135	20170.4643464152\\
%137	20158.9435350462\\
%139	20138.3196151305\\
%141	20100.9434460445\\
%143	20092.6581368683\\
%145	20042.0194582237\\
%147	20031.5114047339\\
%149	20012.8739986706\\
%151	19979.3926783265\\
%153	19971.8537079642\\
%155	19926.5132522682\\
%157	19917.2815534433\\
%159	19900.6854319737\\
%161	19870.554412678\\
%163	19863.8471735115\\
%165	19822.7698173857\\
%167	19814.2488592552\\
%169	19799.0303830585\\
%171	19771.6194956176\\
%173	19765.4449371633\\
%175	19728.2906193063\\
%177	19720.7161815055\\
%179	19707.0532121572\\
%181	19682.1969420638\\
%183	19676.6496842257\\
%185	19642.6277740344\\
%187	19635.5666870875\\
%189	19622.8891924741\\
%191	19599.9910859296\\
%193	19594.8330883711\\
%195	19563.7812618492\\
%197	19557.4418552111\\
%199	19545.972627312\\
%};
%\addlegendentry{R-Broyden};

\addplot [color=color_BFGS,\linestylelimited,line width=1.5pt]
  table[row sep=crcr]{%
1	362679.178539387\\
3	139455.679423477\\
5	64769.0654111213\\
7	45828.0703134029\\
9	35889.0379067751\\
11	31888.0395781502\\
13	29088.2561597705\\
15	27522.4657766175\\
17	26437.1134135777\\
19	25633.6980105906\\
21	25032.0552074305\\
23	24413.3874490751\\
25	23994.324436893\\
27	23644.6342407311\\
29	23327.6413000296\\
31	23022.2414609356\\
33	22768.0586367487\\
35	22545.5816668014\\
37	22352.9496926665\\
39	22164.8347208423\\
41	21986.4830099313\\
43	21845.0992136381\\
45	21702.392863858\\
47	21549.9840946883\\
49	21406.2933365795\\
51	21280.9553767991\\
53	21184.0475087146\\
55	21066.5462402695\\
57	20965.1675843663\\
59	20860.5515916569\\
61	20780.6571513468\\
63	20689.9916995417\\
65	20612.5912024234\\
67	20527.2546729277\\
69	20460.5550960638\\
71	20386.5159666548\\
73	20323.1866557929\\
75	20253.4026735541\\
77	20196.7912855235\\
79	20138.5171618483\\
81	20088.6322194461\\
83	20031.6056870854\\
85	19984.0232703109\\
87	19935.0044760827\\
89	19892.7721336232\\
91	19845.7190148815\\
93	19805.3097773481\\
95	19763.0370109415\\
97	19726.9770662153\\
99	19688.2423887885\\
101	19654.4548181656\\
103	19618.8480892877\\
105	19587.9338268768\\
107	19555.7535514283\\
109	19526.8558811785\\
111	19495.4087909095\\
113	19467.3531978746\\
115	19438.3057043683\\
117	19412.2673447016\\
119	19384.7967181486\\
121	19359.9683903025\\
123	19333.9633136687\\
125	19310.7153132242\\
127	19286.4101896788\\
129	19264.2800692359\\
131	19240.998856257\\
133	19219.9210303157\\
135	19197.978559737\\
137	19177.9465504996\\
139	19156.5864006082\\
141	19136.9843053399\\
143	19116.3202131739\\
145	19097.6172467235\\
147	19078.1759415318\\
149	19060.5189669093\\
151	19041.9976080074\\
153	19025.0457331176\\
155	19007.1555624596\\
157	18990.7012001493\\
159	18973.4143962211\\
161	18957.6646412663\\
163	18941.3669501784\\
165	18926.5686967699\\
167	18911.0669217321\\
169	18896.8091462818\\
171	18881.7652354224\\
173	18867.9866904234\\
175	18853.6667430928\\
177	18840.5618986875\\
179	18826.9126390511\\
181	18814.3026363103\\
183	18801.0914277902\\
185	18788.8478218289\\
187	18776.0251060678\\
189	18764.1547810739\\
191	18751.8222252543\\
193	18740.4624430529\\
195	18728.7579167316\\
197	18717.9419655642\\
199	18706.731717289\\
};
\addlegendentry{ZeroFPR(L-BFGS)};

\end{axis}
\end{tikzpicture}%


==> TeX/Tikz/MatComp/MatComp_5.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
% \definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
% \definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
% \definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
% \definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}

\begin{axis}[%
% width=1.2in,
% height=1.0in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=100,
ymin=1e4,
ymax=1e5,
xlabel={number of SVDs},
ylabel={$\varphi(x^k)$},
xmajorgrids,
ymajorgrids,
axis background/.style={fill=white},
legend style={legend cell align=left,align=left,draw=white!15!black}
]
\addplot [color=color_FBS,line width=1.5pt]
  table[row sep=crcr]{%
1	402264.934989514\\
2	239049.009689886\\
3	176177.981301077\\
4	142250.45195292\\
5	121012.173106579\\
6	106499.108993905\\
7	95977.2799106784\\
8	88013.0422233357\\
9	81782.5078289523\\
10	76779.2680167345\\
11	72675.4463659051\\
12	69249.7231788151\\
13	66347.4914285023\\
14	63857.5926166152\\
15	61698.1221154543\\
16	59807.4403766549\\
17	58138.2962371132\\
18	56653.8767927927\\
19	55325.0868045148\\
20	54128.6341249836\\
21	53045.6562568842\\
22	52060.718028613\\
23	51161.0687100032\\
24	50336.0836600742\\
25	49576.8393008615\\
26	48875.7858050608\\
27	48226.492337109\\
28	47623.4468138313\\
29	47061.8970862951\\
30	46537.72391265\\
31	46047.3385613541\\
32	45587.5996646134\\
33	45155.7452402203\\
34	44749.3367569436\\
35	44366.212830926\\
36	44004.4506757506\\
37	43662.3338344171\\
38	43338.3250313555\\
39	43031.0432211943\\
40	42739.2440960076\\
41	42461.8034572334\\
42	42197.7029719491\\
43	41946.01792295\\
44	41705.9066334395\\
45	41476.6013041907\\
46	41257.4000469242\\
47	41047.65993468\\
48	40846.7909200503\\
49	40654.2504966563\\
50	40469.5389993382\\
51	40292.195455045\\
52	40121.793910051\\
53	39957.9401704343\\
54	39800.2689021582\\
55	39648.4410449571\\
56	39502.1415008068\\
57	39361.0770633027\\
58	39224.9745589313\\
59	39093.5791751777\\
60	38966.6529537617\\
61	38843.9734301545\\
62	38725.3324029615\\
63	38610.5348188455\\
64	38499.397760457\\
65	38391.7495263783\\
66	38287.4287934185\\
67	38186.2838527493\\
68	38088.1719123668\\
69	37992.9584592336\\
70	37900.5166752096\\
71	37810.7269015406\\
72	37723.4761472498\\
73	37638.6576372838\\
74	37556.1703967093\\
75	37475.918867646\\
76	37397.8125559703\\
77	37321.7657051235\\
78	37247.6969946347\\
79	37175.5292612004\\
80	37105.1892403834\\
81	37036.6073271752\\
82	36969.71735384\\
83	36904.4563836066\\
84	36840.7645189078\\
85	36778.5847229908\\
86	36717.8626538263\\
87	36658.5465093433\\
88	36600.5868831017\\
89	36543.9366295969\\
90	36488.5507384554\\
91	36434.3862168503\\
92	36381.4019795195\\
93	36329.5587458223\\
94	36278.8189433173\\
95	36229.1466173892\\
96	36180.5073464871\\
97	36132.8681625762\\
98	36086.1974764343\\
99	36040.4650074547\\
100	35995.6417176443\\
101	35951.6997495284\\
102	35908.6123676978\\
103	35866.3539037529\\
104	35824.8997044183\\
105	35784.2260826186\\
106	35744.3102713216\\
107	35705.1303799693\\
108	35666.6653533305\\
109	35628.8949326208\\
110	35591.7996187454\\
111	35555.360637534\\
112	35519.5599068423\\
113	35484.3800054054\\
114	35449.804143337\\
115	35415.8161341731\\
116	35382.4003683692\\
117	35349.5417881632\\
118	35317.2258637234\\
119	35285.4385705065\\
120	35254.1663677552\\
121	35223.3961780695\\
122	35193.1153679901\\
123	35163.3117295366\\
124	35133.9734626463\\
125	35105.0891584639\\
126	35076.6477834338\\
127	35048.6386641519\\
128	35021.0514729339\\
129	34993.8762140631\\
130	34967.103210679\\
131	34940.7230922744\\
132	34914.7267827664\\
133	34889.1054891132\\
134	34863.8506904472\\
135	34838.9541276971\\
136	34814.407793674\\
137	34790.2039235989\\
138	34766.3349860466\\
139	34742.7936742882\\
140	34719.5728980085\\
141	34696.6657753835\\
142	34674.0656254964\\
143	34651.7659610783\\
144	34629.7604815567\\
145	34608.0430663959\\
146	34586.6077687171\\
147	34565.4488091833\\
148	34544.5605701371\\
149	34523.9375899791\\
150	34503.574557776\\
151	34483.4663080873\\
152	34463.6078160002\\
153	34443.9941923642\\
154	34424.6206792153\\
155	34405.4826453808\\
156	34386.5755822583\\
157	34367.8950997582\\
158	34349.4369224064\\
159	34331.1968855954\\
160	34313.1709319814\\
161	34295.3551080178\\
162	34277.7455606222\\
163	34260.3385339678\\
164	34243.1303663965\\
165	34226.1174874473\\
166	34209.2964149951\\
167	34192.6637524954\\
168	34176.2161863309\\
169	34159.9504832541\\
170	34143.8634879248\\
171	34127.952120535\\
172	34112.2133745203\\
173	34096.644314354\\
174	34081.2420734184\\
175	34066.0038519524\\
176	34050.9269150725\\
177	34036.0085908613\\
178	34021.2462685246\\
179	34006.6373966116\\
180	33992.1794812976\\
181	33977.8700847245\\
182	33963.7068233994\\
183	33949.6873666475\\
184	33935.8094351167\\
185	33922.0707993344\\
186	33908.4692783109\\
187	33895.0027381906\\
188	33881.6690909483\\
189	33868.4662931276\\
190	33855.3923446222\\
191	33842.4452874964\\
192	33829.623204844\\
193	33816.9242196849\\
194	33804.3464938969\\
195	33791.8882271824\\
196	33779.5476560678\\
197	33767.3230529342\\
198	33755.2127250806\\
199	33743.2150138154\\
200	33731.3282935763\\
};
%\addlegendentry{fbs,basic,none,none};

%\addplot [color=mycolor2,solid]
%  table[row sep=crcr]{%
%1	416469.288240047\\
%3	182893.576143356\\
%5	101204.754793551\\
%7	78246.2645104711\\
%9	64274.5015858543\\
%11	56424.5301167338\\
%13	51018.6764966976\\
%15	47267.6075656046\\
%17	44437.3877264418\\
%19	42478.3258701175\\
%21	40876.0666057479\\
%23	39665.2844854488\\
%25	38697.1053337238\\
%27	37926.6767614353\\
%29	37279.8129118733\\
%31	36760.7835645\\
%33	36311.7576169169\\
%35	35926.1361218972\\
%37	35588.387189198\\
%39	35293.1811882544\\
%41	35026.2072103319\\
%43	34791.5974945024\\
%45	34581.6668208493\\
%47	34393.3055591626\\
%49	34223.2176802585\\
%51	34070.4876766146\\
%53	33929.9764828823\\
%55	33801.1273835298\\
%57	33682.506331439\\
%59	33572.7676629115\\
%61	33470.6387599138\\
%63	33376.5017973043\\
%65	33289.1398145576\\
%67	33207.893223022\\
%69	33132.3668076542\\
%71	33062.0320062512\\
%73	32995.9108555765\\
%75	32933.8183591308\\
%77	32875.3963931851\\
%79	32820.1998458288\\
%81	32768.0069887233\\
%83	32718.8100147602\\
%85	32672.2655981418\\
%87	32628.1743668814\\
%89	32586.4290422269\\
%91	32546.8010532237\\
%93	32509.01194311\\
%95	32472.9788051677\\
%97	32438.5577427352\\
%99	32405.5762237848\\
%101	32373.9674552507\\
%103	32343.6994012736\\
%105	32314.6547604006\\
%107	32286.7763033703\\
%109	32260.0397115151\\
%111	32234.3666924407\\
%113	32209.6791961736\\
%115	32185.9557643777\\
%117	32163.1430504471\\
%119	32141.1751346037\\
%121	32120.0262083726\\
%123	32099.6699430891\\
%125	32080.0513662127\\
%127	32061.1410691635\\
%129	32042.9200045605\\
%131	32025.3464511897\\
%133	32008.3845794803\\
%135	31992.0178216065\\
%137	31976.2138999707\\
%139	31960.9358455392\\
%141	31946.1621498996\\
%143	31931.8661714853\\
%145	31918.0094711773\\
%147	31904.5646750147\\
%149	31891.5073529391\\
%151	31878.8035782354\\
%153	31866.4252208362\\
%155	31854.3538324194\\
%157	31842.5657463057\\
%159	31831.0389031043\\
%161	31819.7614597907\\
%163	31808.7207734033\\
%165	31797.9015675968\\
%167	31787.2962981762\\
%169	31776.8995514542\\
%171	31766.7019828202\\
%173	31756.6982243335\\
%175	31746.8872223834\\
%177	31737.2645350496\\
%179	31727.826425621\\
%181	31718.5735715681\\
%183	31709.504827207\\
%185	31700.6171167169\\
%187	31691.9105561846\\
%189	31683.3849229159\\
%191	31675.0369599157\\
%193	31666.8647150457\\
%195	31658.8670866052\\
%197	31651.0400661754\\
%199	31643.379322076\\
%};
%\addlegendentry{zerofpr,,lbroyden,backtracking-nm};

%\addplot [color=mycolor3,solid]
%  table[row sep=crcr]{%
%1	416469.28824004\\
%3	182893.576143342\\
%5	101204.75479355\\
%7	78410.7310667327\\
%9	63834.3404360398\\
%11	55953.3153377264\\
%13	53709.1775699792\\
%15	44673.0968137377\\
%17	41598.4540000651\\
%19	40118.315560035\\
%21	38754.5850473474\\
%23	38471.9793053319\\
%25	37000.736386745\\
%27	36599.0695147838\\
%29	36206.0214462007\\
%31	35684.8463525323\\
%33	35570.9780323537\\
%35	34997.5431033899\\
%37	34881.1851347109\\
%39	34714.1736840255\\
%41	34452.1422328739\\
%43	34397.1901394935\\
%45	34064.8189527177\\
%47	33993.7630476534\\
%49	33889.308991541\\
%51	33710.4476814168\\
%53	33673.6517552243\\
%55	33468.2100045504\\
%57	33428.9681822475\\
%59	33363.8499110481\\
%61	33250.3929121683\\
%63	33226.8854322324\\
%65	33080.3541914469\\
%67	33050.0197964411\\
%69	33001.8176061895\\
%71	32919.316406431\\
%73	32900.9216694159\\
%75	32795.7929234014\\
%77	32775.8518248654\\
%79	32741.2880347965\\
%81	32679.8479138603\\
%83	32666.7758913476\\
%85	32584.4764246437\\
%87	32567.4055875683\\
%89	32539.3169615162\\
%91	32491.1794591683\\
%93	32480.1069450795\\
%95	32416.2880710053\\
%97	32404.1640917348\\
%99	32382.663360467\\
%101	32343.8974106616\\
%103	32335.5662425597\\
%105	32282.7846242152\\
%107	32271.7926596227\\
%109	32253.3477705534\\
%111	32221.6032866588\\
%113	32214.2058969774\\
%115	32171.3848766882\\
%117	32163.2362826807\\
%119	32148.6076769849\\
%121	32122.0088579151\\
%123	32116.2481863246\\
%125	32079.5614101147\\
%127	32071.8951347921\\
%129	32058.8747934123\\
%131	32036.3802502852\\
%133	32031.0966463727\\
%135	32000.4101225022\\
%137	31994.5619623438\\
%139	31983.9810505074\\
%141	31964.6230980025\\
%143	31960.404800855\\
%145	31933.4078748184\\
%147	31927.7490355282\\
%149	31918.0563513294\\
%151	31901.2489628421\\
%153	31897.2793105075\\
%155	31874.1559649632\\
%157	31869.7440259574\\
%159	31861.7162273515\\
%161	31846.9547737115\\
%163	31843.7227456515\\
%165	31822.9452963209\\
%167	31818.5792734617\\
%169	31811.0538040734\\
%171	31797.9626359696\\
%173	31794.8577154091\\
%175	31776.7257142855\\
%177	31773.2640163445\\
%179	31766.9384120857\\
%181	31755.2600568363\\
%183	31752.6933236757\\
%185	31736.1302081653\\
%187	31732.6435220904\\
%189	31726.6054238594\\
%191	31716.0757162198\\
%193	31713.5697583045\\
%195	31698.9056119455\\
%197	31696.1055563291\\
%199	31690.972624312\\
%};
%\addlegendentry{zerofpr,,rbroyden,backtracking-nm};

\addplot [color=color_BFGS,\linestylelimited,line width=1.5pt]
  table[row sep=crcr]{%
1	416469.288240046\\
3	182893.576143364\\
5	84663.4665193536\\
7	60163.1620682689\\
9	48695.1373856593\\
11	43778.4621620762\\
13	39997.4445350378\\
15	38546.3146780015\\
17	36994.3720423755\\
19	36131.1909528283\\
21	35564.9130117609\\
23	34920.4953873076\\
25	34517.9640787348\\
27	34212.5891405121\\
29	33885.9313686242\\
31	33659.8709252833\\
33	33473.9337124391\\
35	33297.7382773868\\
37	33127.233989209\\
39	32995.1806406458\\
41	32866.5389744885\\
43	32762.2532280848\\
45	32654.2432022632\\
47	32575.4975018151\\
49	32492.275228278\\
51	32426.374794502\\
53	32354.6730073269\\
55	32295.6509266614\\
57	32231.3526248848\\
59	32180.0802041327\\
61	32122.0437329444\\
63	32078.8177055314\\
65	32033.8206098244\\
67	31999.4986660513\\
69	31957.7671029987\\
71	31926.0102181304\\
73	31893.1285706332\\
75	31866.420631998\\
77	31836.055574218\\
79	31810.2743105616\\
81	31783.3257249124\\
83	31761.3281203156\\
85	31737.5874000769\\
87	31717.0542525035\\
89	31695.0742002118\\
91	31676.4317309136\\
93	31656.5568099649\\
95	31639.7212741189\\
97	31621.0229898664\\
99	31605.4092485684\\
101	31588.8080337421\\
103	31574.3412258113\\
105	31558.8563787062\\
107	31545.6727835847\\
109	31531.9799230239\\
111	31520.0478932689\\
113	31507.470692579\\
115	31496.1921472482\\
117	31484.5321225524\\
119	31474.016441061\\
121	31463.13189256\\
123	31453.1770173954\\
125	31442.8316738814\\
127	31433.4313258831\\
129	31423.9023477261\\
131	31415.158750227\\
133	31406.2463577101\\
135	31397.9295894215\\
137	31389.3880463278\\
139	31381.346154258\\
141	31373.1146058948\\
143	31365.3418784601\\
145	31357.4644315028\\
147	31350.0083474434\\
149	31342.4580704132\\
151	31335.2397140419\\
153	31327.8956041092\\
155	31320.8408954959\\
157	31313.6715888924\\
159	31306.8071206731\\
161	31299.8526944796\\
163	31293.2617240659\\
165	31286.5876401229\\
167	31280.3134980742\\
169	31273.8999689917\\
171	31267.8860649825\\
173	31261.7099506046\\
175	31255.9473322494\\
177	31250.0720694001\\
179	31244.5739558786\\
181	31238.9666279275\\
183	31233.641510293\\
185	31228.1803668708\\
187	31222.9272235472\\
189	31217.5353197746\\
191	31212.3216094993\\
193	31206.9838206006\\
195	31201.8239584419\\
197	31196.5271291789\\
199	31191.4113556315\\
};
%\addlegendentry{zerofpr,,lbfgs,backtracking-nm};

\end{axis}
\end{tikzpicture}%

